CheckSel: Efficient and Accurate Data-valuation Through Online Checkpoint Selection

Data valuation and subset selection have emerged as valuable tools for application-specific selection of important training data. However, the efficiency-accuracy tradeoffs of state-of-the-art methods hinder their widespread application to many AI workflows. In this paper, we propose a novel 2-phase solution to this problem. Phase 1 selects representative checkpoints from an SGD-like training algorithm, which are used in phase-2 to estimate the approximate training data values, e.g. decrease in validation loss due to each training point. A key contribution of this paper is CheckSel, an Orthogonal Matching Pursuit-inspired online sparse approximation algorithm for checkpoint selection in the online setting, where the features are revealed one at a time. Another key contribution is the study of data valuation in the domain adaptation setting, where a data value estimator obtained using checkpoints from training trajectory in the source domain training dataset is used for data valuation in a target domain training dataset. Experimental results on benchmark datasets show the proposed algorithm outperforms recent baseline methods by up to 30% in terms of test accuracy while incurring a similar computational burden, for both standalone and domain adaptation settings.

==> experiment.tex <==
\section{Experiments}
In this section, we evaluate our approach on three datasets - CIFAR10, CIFAR100 and Tinyimagenet using ResNet-18. In Section \ref{sec:add}, we show the effectiveness of the proposed method on addition of instances. Next, in Section \ref{sec:vary}, we show the effect of varying number of selected checkpoints, followed by a comparison of timing profile in Section \ref{sec:time}.

\subsection{Addition of instances}
\label{sec:add}
We compare our method with \textit{UnifSelect} that uniformly selects checkpoints followed by valuating data using \cite{NEURIPS2020_e6385d39}. Owing to the fact that random runs can lead to varying intermediate checkpoints, we execute 10 runs for CIFAR10 and 5 runs for CIFAR100 and Tinyimagenet, while acquiring k(=10) UnifSelect or CheckSelect based checkpoints. Following that, we utilize the above selected checkpoints and compute the score for valuating datapoints. Depending on the obtained values, we select top-$f\%$ data and train the models only on the selected datapoints. We report the average performance difference in accuracies (\textit{CheckSelect-UnifSelect}) in Table \ref{tab:add}. We can observe that CheckSelect performs better across all the datasets for all the fractions, thus signifying the positive impact of selected checkpoints using \textit{CheckSelect}.


\begin{table}
\centering
\caption{Performance difference (\textit{CheckSelect - UnifSelect}) on addition of instances}
\label{tab:add}
\begin{tabular}{ |c|c|c|c| }
 \hline
  \textbf{Frac (f\%)} & \textbf{CIFAR10} & \textbf{CIFAR100} & \textbf{Tinyimagenet} \\
  \hline
 5 & 3.64\% & 0.39\% &  \\ 
 \hline
 20 & 2.75\% & 0.25\%  &  \\ 
 \hline
 35 & 5.8\% & 0.68\% &  \\
 \hline
\end{tabular}
\end{table}

% \begin{table}[]
% \footnotesize
% \caption{Performance comparison on addition of instances in CIFAR10,CIFAR100,Tinyimagenet}
% \label{tab:add}
% \begin{tabular}{|l|p{16mm}|p{16mm}|l|p{16mm}|p{16mm}|l|p{16mm}|p{16mm}|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Frac\\(f\%)\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{CIFAR10}}                                                                                                                                                & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Frac\\(f\%)\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{CIFAR100}}                                                                                                                                               & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Frac\\(f\%)\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{Tinyimagenet}}                                                                                                                                           \\ \cline{2-3} \cline{5-6} \cline{8-9} 
% \multicolumn{1}{|c|}{}                                                                              & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Unif-Sel-\\ TracIn\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Check-Sel-\\ TracIn\end{tabular}}} & \multicolumn{1}{c|}{}                                                                              & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Unif-Sel-\\ TracIn\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Check-Sel-\\ TracIn\end{tabular}}} & \multicolumn{1}{c|}{}                                                                              & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Unif-Sel-\\ TracIn\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Check-Sel-\\ TracIn\end{tabular}}} \\ \hline
% 5                                                                                                   & \begin{tabular}[c]{@{}l@{}}31.87± 4.97\end{tabular}                       & \begin{tabular}[c]{@{}l@{}}35.51±5.89\end{tabular}                         & 5                                                                                                 & \begin{tabular}[c]{@{}l@{}}11.5±1.5\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}11.9±1.5\end{tabular}                         & 20                                                                                                 & \begin{tabular}[c]{@{}l@{}}26.31±1.28\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}26.56±1.52\end{tabular}                               \\ \hline
% 20                                                                                                  & \begin{tabular}[c]{@{}l@{}}59.54±4.13\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}62.29±10.52\end{tabular}                        & 20                                                                                                 & \begin{tabular}[c]{@{}l@{}}±\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}±\end{tabular}                          & 40                                                                                                 & \begin{tabular}[c]{@{}l@{}}36.45±0.63\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}37.16±0.60\end{tabular}                               \\ \hline
% 35                                                                                                  & \begin{tabular}[c]{@{}l@{}}69.36±5.77\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}75.17±10.18\end{tabular}                                                                & 35                                                                                                 & \begin{tabular}[c]{@{}l@{}}54.78±0.81\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}55.46±1.7\end{tabular}                         & 60                                                                                                 & \begin{tabular}[c]{@{}l@{}}40.24±0.95\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}40.6±0.97\end{tabular}                                \\ \hline
% \end{tabular}
% \end{table}



% \begin{table*}
% \footnotesize
% \centering
% \caption{Performance comparison on addition of instances in CIFAR10 (k = 10)}
% \label{tab:perfcomp_cf10}
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Fraction of\\ addition(\%)\end{tabular}} & \textbf{Unif-Sel-TracIn}                                                        & \textbf{Check-Sel-TracIn}                                               \\ \hline
% 5                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}31.87 $\pm$ 4.97\\ (128+70)mins\end{tabular}  & \begin{tabular}[c]{@{}l@{}}35.51 $\pm$ 5.89\\ (137+70)mins\end{tabular}  \\ \hline
% 20                                                                                                                      & \begin{tabular}[c]{@{}l@{}}59.54$\pm$ 4.13\\ (128+70)mins\end{tabular} & \begin{tabular}[c]{@{}l@{}}62.29 $\pm$ 10.52\\ (137+70)mins\end{tabular}     \\ \hline
% 35                                                             & \begin{tabular}[c]{@{}l@{}}69.36$\pm$5.77 \\ (128+70)mins\end{tabular}  & \begin{tabular}[c]{@{}l@{}}75.17$\pm$10.18\\ (137+70)mins\end{tabular}  \\ \hline

% \end{tabular}
% \end{table*}

% \begin{table*}
% \footnotesize
% \centering
% \caption{Performance comparison on addition of instances in CIFAR100 (k = 10)}
% \label{tab:perfcomp_cf100k10}
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Fraction of\\ addition(\%)\end{tabular}} & \textbf{Unif-Sel-TracIn}                                             & \textbf{Check-Sel-TracIn}                                                      \\ \hline
% 15                                                           & \begin{tabular}[c]{@{}l@{}}29.48 $\pm$ 0.83\\ (128+70)mins\end{tabular} & \begin{tabular}[c]{@{}l@{}}31.15 $\pm$ 1.54\\ (137+70)mins\end{tabular} \\ \hline
% 35                                                         & \begin{tabular}[c]{@{}l@{}}54.78$\pm$0.81\\ (128+70)mins\end{tabular} & \begin{tabular}[c]{@{}l@{}}55.46$\pm$1.7\\ (137+70)mins\end{tabular} \\ \hline
% 65                                                         & \begin{tabular}[c]{@{}l@{}}70.63$\pm$0.86\\ (128+70)mins\end{tabular} & \begin{tabular}[c]{@{}l@{}}70.69$\pm$0.55
% \\ (137+70)mins\end{tabular} \\ \hline

% \end{tabular}
% \end{table*}

% \begin{table*}
% \footnotesize
% \centering
% \caption{Performance comparison on addition of instances in Tinyimagenet (k = 10)}
% \label{tab:perfcomp_cf10}
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Fraction of\\ addition(\%)\end{tabular}} & \textbf{Unif-Sel-TracIn}                                              & \textbf{Check-Sel-TracIn}    \\ \hline
% 20                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}26.31$\pm$1.28\\ ()mins\end{tabular}  & \begin{tabular}[c]{@{}l@{}}26.56$\pm$1.52\\ ()mins\end{tabular}  \\ \hline
% 40                                                                                             & \begin{tabular}[c]{@{}l@{}}36.45$\pm$0.63\\ ()mins\end{tabular} & \begin{tabular}[c]{@{}l@{}}37.16$\pm$0.60\\ ()mins\end{tabular}      \\ \hline
% 60                                                             & \begin{tabular}[c]{@{}l@{}}40.24$\pm$0.95\\ ()mins\end{tabular} & \begin{tabular}[c]{@{}l@{}}40.6$\pm$0.97\\ ()mins\end{tabular}      \\ \hline

% \end{tabular}
% \end{table*}

\subsection{Variation in selection of checkpoints}
\label{sec:vary}
We also vary the number of selected checkpoints (k) and show the difference in accuracy performance \textit{(CheckSelect-UnifSelect)} on CIFAR10 in Table \ref{tab:vary}. We can observe that CheckSelect consistently performs better(+ve difference) than UnifSelect across different selected checkpoints. It is to be noted that the \textit{CheckSelect} has a unique solution for each $k$. It can be seen that the difference between the performance of UnifSelect and CheckSelect is more prominent at a lower value of $k$ and increasing fraction of instances. The difference decreases with increasing value of $k$. The observed trend is possibly due to the fact that higher value of $k$, for some runs, leads to selection of some closely spaced checkpoints towards the tail of the training, which might not have a higher reduction loss rate, thus leading to a lower difference with that of uniformly spaced checkpoints.

\begin{table}
\centering
\caption{Performance difference (\textit{CheckSelect - UnifSelect}) in CIFAR10 for varying $k$}
\label{tab:vary}
\begin{tabular}{ |c|c|c|c|}
 \hline
  \textbf{Frac (f\%)} & \textbf{k=3} & \textbf{k=5} & \textbf{k=20} \\
  \hline
 5 & 7.29\% & 4.06\%  & 1.27\%\\ 
 \hline
 20 & 8.86\% & 4.42\% & 2.86\%\\ 
 \hline
 35 & 12.45\% & 8.04\% & 1.45\%\\
 \hline
\end{tabular}
\end{table}

% \begin{table}[]
% \footnotesize
% \caption{Performance comparison on addition of instances in CIFAR10 for varying $k$}
% \label{tab:vary}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Frac\\(f\%)\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{k = 3}}                                                                                                                                                  & \multicolumn{2}{c|}{\textbf{k = 5}}                                                                                                                                                  \\ \cline{2-5} 
% \multicolumn{1}{|c|}{}                                                                              & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Unif-Sel-\\ TracIn\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Check-Sel-\\ TracIn\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Unif-Sel-\\ TracIn\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Check-Sel-\\ TracIn\end{tabular}}} \\ \hline
% 5                                                                                                   & \begin{tabular}[c]{@{}l@{}}30.49±5.79\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}37.79±3.46\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}30.2±5.04\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}34.35±4.3\end{tabular}                          \\ \hline
% 20                                                                                                  & \begin{tabular}[c]{@{}l@{}}58.08±3.54\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}67±7.63\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}57.55±4.15\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}61.98±7.53\end{tabular}                         \\ \hline
% 35                                                                                                  & \begin{tabular}[c]{@{}l@{}}66.36±3.57\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}78.8±9.15\end{tabular}                          & \begin{tabular}[c]{@{}l@{}}66.62±3.83\end{tabular}                        & \begin{tabular}[c]{@{}l@{}}74.66±9.8\end{tabular}                          \\ \hline
% \end{tabular}
% \end{table}

\subsection{Timing profile}
\label{sec:time}
In this section, we also report the time taken by both the methods for k=10 checkpoints. We divide the consumed time into two parts - training time T (during which the checkpoints are selected) and the score evaluation time S. We can observe that CheckSelect takes a small amount of extra time compared to UnifSelect, thus turning out to be equivalent in computational order. It is to be noted that the score evaluation time S is directly proportional to the number of selected checkpoints, while the training time T stays constant.
\begin{table}[h]
\caption{Time consumed by \textit{UnifSelect} and \textit{CheckSelect} for k=10 checkpoints}
\centering
\begin{tabular}{ |c|c|c|c| }
 \hline
  \textbf{Method} & \textbf{CIFAR10} & \textbf{CIFAR100} & \textbf{Tinyimagenet} \\
  \hline
 UnifSelect & (128T +70S )mins & (128T +70S )mins & (9T + 2.1S) hours \\ 
 \hline
 CheckSelect & (137T +70S )mins & (137T +70S )mins & (10.5T + 2.1S) hours \\ 
 \hline
\end{tabular}
\end{table}
% \begin{table*}
% \footnotesize
% \centering
% \caption{Performance comparison on addition of instances in CIFAR10 (k = 3)}
% \label{tab:perfcomp_cf10}
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Fraction of\\ addition(\%)\end{tabular}}  & \textbf{Unif-Sel-TracIn}                                               & \textbf{Check-Sel-TracIn}                                          \\ \hline
% 5                                                                                             & \begin{tabular}[c]{@{}l@{}}30.49 $\pm$ 5.79\\ (128+20)mins\end{tabular}  & \begin{tabular}[c]{@{}l@{}}37.79 $\pm$ 3.46\\ (137+20)mins\end{tabular} \\ \hline
% 20                                                & \begin{tabular}[c]{@{}l@{}}58.08$\pm$ 3.54\\ (128+20)mins\end{tabular}  & \begin{tabular}[c]{@{}l@{}}67 $\pm$ 7.63\\ (137+20)mins\end{tabular}\\ \hline
% 35                                                                           & \begin{tabular}[c]{@{}l@{}}66.36$\pm$3.57 \\ (128+20)mins\end{tabular}  & \begin{tabular}[c]{@{}l@{}}78.8$\pm$9.15\\ (137+20)mins\end{tabular}   \\ \hline

% \end{tabular}
% \end{table*}

% \begin{table*}
% \footnotesize
% \centering
% \caption{Performance comparison on addition of instances in CIFAR10 (k = 5)}
% \label{tab:perfcomp_cf10}
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Fraction of\\ addition(\%)\end{tabular}} & \textbf{Unif-Sel-TracIn}                                                 & \textbf{Check-Sel-TracIn}                                                 \\ \hline
% 5                                                                         & \begin{tabular}[c]{@{}l@{}}30.2 $\pm$ 5.04\\ (128+30)mins\end{tabular}  & \begin{tabular}[c]{@{}l@{}}34.35 $\pm$ 4.3\\ (137+30)mins\end{tabular} \\ \hline
% 20                                                             & \begin{tabular}[c]{@{}l@{}}57.55$\pm$ 4.15\\ (128+30)mins\end{tabular}    & \begin{tabular}[c]{@{}l@{}}61.98 $\pm$ 7.53\\ (137+30)mins\end{tabular}   \\ \hline
% 35                                                             & \begin{tabular}[c]{@{}l@{}}66.62 $\pm$ 3.83 \\ (128+30)mins\end{tabular}  & \begin{tabular}[c]{@{}l@{}}74.66 $\pm$ 9.8\\ (137+30)mins\end{tabular} \\ \hline

% \end{tabular}
% \end{table*}






==> experiment2.tex <==
\section{Experiments}
In this section, we evaluate our approach on three datasets - CIFAR10, CIFAR100, and Tinyimagenet using ResNet-18. In Section \ref{sec:addgreater}, we show the overall effectiveness of the proposed method in data valuation in terms of time and classification accuracies. We follow this discussion with some analytical results to demonstrate the usefulness of the subsets in Section \ref{sec:analyse}. Lastly, in Section \ref{sec:domadapt}, we show its application on domain adaptation using the proposed method on \textit{Office-Home} dataset. 

% \begin{figure}[h!]
%     %\centering
%     %\begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=0.75\columnwidth,height=4cm]{latex/figs/cifar10adds2.pdf}
%     %\caption{Red light before junction}
%     \label{fig:subdiag}
%     %\end{subfigure}
%     \caption{\textbf{Performance on CIFAR10}}
%     \label{fig:subsetdiag}
% \end{figure}

\subsection{Efficient data valuation}
\label{sec:addgreater}
In this section, we study the effectiveness of the proposed algorithm by selecting a subset of the entire dataset under consideration. We show the performance accuracies along with the consumed time when trained on the selected data using the proposed method and baselines. We select \#CP checkpoints using Algorithm \ref{algo:onlineomp}, following which we execute the data selection phase for some pre-defined fraction of data. We show results on 5 methods - Influence Function \cite{koh2017understanding}, TracIn \cite{NEURIPS2020_e6385d39}, TracIn-Simsel (TracIn with Simsel in data selection phase), CheckSel and CheckSel-Simsel(CheckSel with Simsel in data selection phase). While Influence Function \cite{koh2017understanding} depends only on the final trained model, and hence is independent of \#CP, the other baseline and proposed methods are reliant on intermediate checkpoints.

In Table \ref{tab:sametime}, we show the performance of all methods when executed under similar time constraints. We can see that CheckSel and CheckSel-Simsel consistently perform better than the other methods across all the datasets. We also report the difference in accuracy between (a) CheckSel and TracIn and (b) CheckSel-Simsel and TracIn-Simsel and can observe that CheckSel performs by a maximum margin of more than 35\% than TracIn on CIFAR10.

Next, in Table \ref{tab:perftime}, we show a consolidated result for selecting a subset of 10\% data across three datasets. We do a hyperparameter search over \#CP for each dataset and report their best accuracies along with time taken for each of the methods. The best performing accuracies are highlighted in bold. We can also observe that the second best performing accuracy is less than a margin of 1\%. We divide the timing profile into three components: training time on whole dataset, checkpoint selection time during training (\textbf{CheckSel Time}) applicable for CheckSel and its variant, data valuation and subset selection time (\textbf{DV/SS Time}) applicable for all. Various sub-parts of these components will be holding valid for the different methods.

We show that the proposed method CheckSel or its variant CheckSel-Simsel surpasses the baselines Influence Function \cite{koh2017understanding} and TracIn \cite{NEURIPS2020_e6385d39} by a large margin in the classification task. The method TracIn-Simsel uses Algorithm \ref{algo:simset} to select instances in the data selection phase, post the method of uniformly selecting checkpoints. We can observe that TracIn-Simsel also performs better than TracIn, where the data selection phase involves computing the Tracin \cite{NEURIPS2020_e6385d39} scores using uniformly selected checkpoints. Hence, we can see that the valuation methods CheckSel and CheckSel-Simsel outperform all the baselines across all the datasets.

\begin{table}[]
\footnotesize
\caption{Performance comparison in comparable time consumption}
\label{tab:sametime}
\centering
\begin{tabular}{|lllll|}
\hline
\multicolumn{1}{|l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Infl\\ Func\end{tabular}}} & \multicolumn{1}{l|}{\textbf{TracIn}} & \multicolumn{1}{l||}{\textbf{CheckSel}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}TracIn-\\ Simsel\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ Simsel\end{tabular}} \\ \hline
\multicolumn{5}{|l|}{CIFAR10 (10\% \#CP = 10)}                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|l|}{59.9}                                                         & \multicolumn{1}{l|}{44.13}           & \multicolumn{1}{l||}{\textbf{79.93} (\textbf{\textcolor{blue}{35.8}})}             & \multicolumn{1}{l|}{78.63}                                                             & 79.6 (0.97)                                                                \\ \hline \hline
\multicolumn{5}{|l|}{CIFAR100 (10\% \#CP = 10)}                                                                                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|l|}{21.82}                                                        & \multicolumn{1}{l|}{21.48}           & \multicolumn{1}{l||}{35.48 (14)}             & \multicolumn{1}{l|}{33.96}                                                             & \textbf{35.76} (1.8)                                                               \\ \hline \hline
\multicolumn{5}{|l|}{Tinyimagenet (10\% \#CP = 10)}                                                                                                                                                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{11.74}                                                             & \multicolumn{1}{l|}{20.62}           & \multicolumn{1}{l||}{28.98 (8.36)}             & \multicolumn{1}{l|}{23.46}                                                             & \textbf{29.18} (5.72)                                                               \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\footnotesize
\centering
\caption{Best Performance and Time (in hours) comparison}
\label{tab:perftime}
\begin{tabular}{|llllll|}
\hline
\multicolumn{1}{|l|}{\textbf{Aspects}}                                                    & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Infl}\\ \textbf{Func}\end{tabular}} & \multicolumn{1}{l|}{\textbf{TracIn}} & \multicolumn{1}{l||}{\textbf{CheckSel}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{TracIn}\\ \textbf{Simsel}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\textbf{Checksel}\\ \textbf{Simsel}\end{tabular} \\ \hline
\multicolumn{6}{|l|}{Tinyimagenet(10\%, \#CP = 20)}                                                                                                                                                                                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Test\\ Acc\end{tabular}}      & \multicolumn{1}{l|}{11.74}                                               & \multicolumn{1}{l|}{22.84}  & \multicolumn{1}{l||}{29.44}    & \multicolumn{1}{l|}{23.56}                                                   & \textbf{29.52}                                                    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Total\\ Time\end{tabular}}    & \multicolumn{1}{l|}{11.3}                                                & \multicolumn{1}{l|}{12.91}  & \multicolumn{1}{l||}{12.01}    & \multicolumn{1}{l|}{13.1}                                                    & 12.2                                                      \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel\\ Time\end{tabular}} & \multicolumn{1}{l|}{-}                                                   & \multicolumn{1}{l|}{-}      & \multicolumn{1}{l||}{1.5}      & \multicolumn{1}{l|}{-}                                                       & 1.5                                                       \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}DV/SS\\ Time\end{tabular}}    & \multicolumn{1}{l|}{2.7}                                                 & \multicolumn{1}{l|}{4.3}    & \multicolumn{1}{l||}{1.9}      & \multicolumn{1}{l|}{4.49}                                                    & 2.09                                                      \\ \hline
\multicolumn{6}{|l|}{CIFAR10(10\%, \#CP = 10)}                                                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Test\\ Acc\end{tabular}}      & \multicolumn{1}{l|}{59.9}                                                & \multicolumn{1}{l|}{44.13}  & \multicolumn{1}{l||}{\textbf{79.93}}    & \multicolumn{1}{l|}{78.63}                                                   & 79.6                                                      \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Total\\ Time\end{tabular}}    & \multicolumn{1}{l|}{4.0}                                                 & \multicolumn{1}{l|}{3.13}   & \multicolumn{1}{l||}{3.33}     & \multicolumn{1}{l|}{3.29}                                                    & 3.49                                                      \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel\\ Time\end{tabular}} & \multicolumn{1}{l|}{-}                                                   & \multicolumn{1}{l|}{-}      & \multicolumn{1}{l||}{0.3}      & \multicolumn{1}{l|}{-}                                                       & 0.3                                                       \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}DV/SS\\ Time\end{tabular}}    & \multicolumn{1}{l|}{2.0}                                                 & \multicolumn{1}{l|}{1.0}    & \multicolumn{1}{l||}{0.9}      & \multicolumn{1}{l|}{1.16}                                                    & 1.06                                                      \\ \hline
\multicolumn{6}{|l|}{CIFAR100(10\%, \#CP = 5)}                                                                                                                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Test\\ Acc\end{tabular}}      & \multicolumn{1}{l|}{21.82}                                               & \multicolumn{1}{l|}{22.04}  & \multicolumn{1}{l||}{35.28}    & \multicolumn{1}{l|}{35.44}                                                   & \textbf{36.6}                                                      \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Total\\ Time\end{tabular}}    & \multicolumn{1}{l|}{4.0}                                                 & \multicolumn{1}{l|}{2.84}   & \multicolumn{1}{l||}{3.6}      & \multicolumn{1}{l|}{3.01}                                                    & 3.76                                                      \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel\\ Time\end{tabular}} & \multicolumn{1}{l|}{-}                                                   & \multicolumn{1}{l|}{-}      & \multicolumn{1}{l||}{0.4}      & \multicolumn{1}{l|}{-}                                                       & 0.4                                                       \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}DV/SS\\ Time\end{tabular}}    & \multicolumn{1}{l|}{2.0}                                                 & \multicolumn{1}{l|}{0.54}   & \multicolumn{1}{l||}{0.9}      & \multicolumn{1}{l|}{0.71}                                                    & 1.06                                                      \\ \hline
\end{tabular}
\end{table}

% \begin{table}[]
% \footnotesize
% \centering
% \caption{Best Performance and Time comparison}
% \label{tab:perftime}
% \begin{tabular}{|lllll|}
% \hline
% \multicolumn{1}{|l|}{\textbf{Method}}                                            & \multicolumn{1}{l|}{\textbf{Test Acc}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Total\\ Time\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Checksel\\ Time\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}DV/SS\\ Time\end{tabular}} \\ \hline
% \multicolumn{5}{|l|}{CIFAR10 (10\%, \#CP = 10)}                                                                                                                                                                                                                                                                                                             \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Infl\\ Func\end{tabular}}        & \multicolumn{1}{l|}{59.9}              & \multicolumn{1}{l|}{2.0}                    & \multicolumn{1}{l|}{-}                                                                  & \multicolumn{1}{l|}{-}                                                                                           \\ \hline
% \multicolumn{1}{|l|}{TracIn}                                                     & \multicolumn{1}{l|}{44.13}             & \multicolumn{1}{l|}{\textbf{3.13}}                & \multicolumn{1}{l|}{-}                                                                  & 1.0                                                                                          \\ \hline
% \multicolumn{1}{|l|}{CheckSel}                                                   & \multicolumn{1}{l|}{{\textbf{79.93}}}             & \multicolumn{1}{l|}{3.33}              & \multicolumn{1}{l|}{0.3}                                                                & 0.9                                                                                        \\ \hline \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}TracIn-\\ SimSel\end{tabular}}   & \multicolumn{1}{l|}{78.63}              & \multicolumn{1}{l|}{\textbf{3.29}}                & \multicolumn{1}{l|}{-}                                                                  & 1.16                                                                                       \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ SimSel\end{tabular}} & \multicolumn{1}{l|}{\textcolor{blue}{\textbf{79.6}}}              & \multicolumn{1}{l|}{3.49}                & \multicolumn{1}{l|}{0.3}                                                                & 1.06                                                                                       \\ \hline \hline \hline
% \multicolumn{5}{|l|}{CIFAR100 (10\%, \#CP = 5)}                                                                                                                                                                                                                                                                                                             \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Infl\\ Func\end{tabular}}        & \multicolumn{1}{l|}{21.82}              & \multicolumn{1}{l|}{2.0}                    & \multicolumn{1}{l|}{-}                                                                  & \multicolumn{1}{l|}{-}                                                                                           \\ \hline
% \multicolumn{1}{|l|}{TracIn}                                                     & \multicolumn{1}{l|}{22.04}             & \multicolumn{1}{l|}{\textbf{2.84}}                & \multicolumn{1}{l|}{-}                                                                  & 0.54                                                                                          \\ \hline
% \multicolumn{1}{|l|}{CheckSel}                                                   & \multicolumn{1}{l|}{\textcolor{blue}{\textbf{35.28}}}             & \multicolumn{1}{l|}{3.6}                & \multicolumn{1}{l|}{0.4}                                                                & 0.9                                                                                        \\ \hline \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}TracIn-\\ SimSel\end{tabular}}   & \multicolumn{1}{l|}{35.44}              & \multicolumn{1}{l|}{3.01}                & \multicolumn{1}{l|}{-}                                                                  & 0.71                                                                                       \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ SimSel\end{tabular}} & \multicolumn{1}{l|}{\textbf{36.6}}              & \multicolumn{1}{l|}{3.76}                & \multicolumn{1}{l|}{0.4}                                                                & 1.06                                                                                       \\ \hline \hline \hline
% \multicolumn{5}{|l|}{TinyImageNet (10\%, \#CP = 20)}                                                                                                                                                                                                                                                                                                             \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Infl\\ Func\end{tabular}}        & \multicolumn{1}{l|}{11.74}              & \multicolumn{1}{l|}{2.7}                    & \multicolumn{1}{l|}{-}                                                                  & \multicolumn{1}{l|}{-}                                                                                           \\ \hline
% \multicolumn{1}{|l|}{TracIn}                                                     & \multicolumn{1}{l|}{22.84}             & \multicolumn{1}{l|}{12.91}                & \multicolumn{1}{l|}{-}                                                                  & 4.3                                                                                          \\ \hline
% \multicolumn{1}{|l|}{CheckSel}                                                   & \multicolumn{1}{l|}{\textcolor{blue}{\textbf{29.44}}}             & \multicolumn{1}{l|}{\textbf{12.01}}                & \multicolumn{1}{l|}{1.5}                                                                & 1.9                                                                                        \\ \hline \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}TracIn-\\ SimSel\end{tabular}}   & \multicolumn{1}{l|}{23.56}              & \multicolumn{1}{l|}{13.1}                & \multicolumn{1}{l|}{-}                                                                  & 4.49                                                                                       \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ SimSel\end{tabular}} & \multicolumn{1}{l|}{\textbf{29.52}}              & \multicolumn{1}{l|}{\textbf{12.2}}                & \multicolumn{1}{l|}{1.5}                                                                & 2.09                                                                                        \\ \hline
% \end{tabular}
% \end{table}

We also show a variance across checkpoints (\#CP) and fractions of selected data in Figure \ref{fig:varyperf}. We compare the accuracies between (a) CheckSel and TracIn ,and (b) CheckSel-Simsel and TracIn-Simsel and can clearly observe that CheckSel and CheckSel-Simsel outperform the corresponding compared method. It can also be seen that the accuracy difference between the respective methods reduces with increasing fraction of subsets.

While reporting the consumed data valuation/subset selection time (DV/SS) in Figure \ref{fig:varytime1}, we can see that with increasing value of checkpoints (\#CP), the time increases proportionally for TracIn and TracIn-Simsel. However, CheckSel and CheckSel-Simsel have similar value across all variations of checkpoints. This is because in CheckSel, the score of all training points are not computed using all the selected checkpoints but only on the checkpoint associated with that training datapoint. Hence, the valuation time for CheckSel does not depend upon \#CP. The overhead component of checkpoint selection time (\textbf{CheckSel Time}) in variants of CheckSel is also marginally higher than the normal training time as seen in Table \ref{tab:perftime}. We have added the timing profiles for the other two datasets in the Supplementary material. Overall, CheckSel or CheckSel-Simsel are efficient and scalable compared to TracIn or TracIn-Simsel. Owing to the fact that our primary contribution lies in selecting checkpoints and CheckSel-Simsel performs as good as CheckSel, we present the results ahead using CheckSel.



% \begin{table}[]
% \footnotesize
% \centering
% \caption{Performance and Time comparison for subset selection}
% \label{tab:perftime}
% \begin{tabular}{|lllll|}
% \hline
% \multicolumn{1}{|l|}{\textbf{Method}}                                            & \multicolumn{1}{l|}{\textbf{Test Acc}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Total\\ Time\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Checksel\\ Time\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}DV/SS\\ Time\end{tabular}} \\ \hline
% \multicolumn{5}{|l|}{CIFAR10 (10\%, \#CP = 20)}                                                                                                                                                                                                                                                                                                             \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Infl\\ Func\end{tabular}}        & \multicolumn{1}{l|}{59.9}              & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{-}                                                                  & \multicolumn{1}{l|}{-}                                                                                           \\ \hline
% \multicolumn{1}{|l|}{TracIn}                                                     & \multicolumn{1}{l|}{44.73}             & \multicolumn{1}{l|}{4.13}                & \multicolumn{1}{l|}{-}                                                                  & 2                                                                                          \\ \hline
% \multicolumn{1}{|l|}{CheckSel}                                                   & \multicolumn{1}{l|}{\textcolor{blue}{\textbf{79.33}}}             & \multicolumn{1}{l|}{\textbf{3.33}}                & \multicolumn{1}{l|}{0.3}                                                                & 0.9                                                                                        \\ \hline \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}TracIn-\\ SimSel\end{tabular}}   & \multicolumn{1}{l|}{76.9}              & \multicolumn{1}{l|}{4.29}                & \multicolumn{1}{l|}{-}                                                                  & 2.16                                                                                       \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ SimSel\end{tabular}} & \multicolumn{1}{l|}{\textbf{79.7}}              & \multicolumn{1}{l|}{3.49}                & \multicolumn{1}{l|}{0.3}                                                                & 1.06                                                                                       \\ \hline \hline \hline
% \multicolumn{5}{|l|}{CIFAR100 (10\%, \#CP = 20)}                                                                                                                                                                                                                                                                                                             \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Infl\\ Func\end{tabular}}        & \multicolumn{1}{l|}{21.82}              & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{-}                                                                  & \multicolumn{1}{l|}{-}                                                                                           \\ \hline
% \multicolumn{1}{|l|}{TracIn}                                                     & \multicolumn{1}{l|}{19.44}             & \multicolumn{1}{l|}{4.46}                & \multicolumn{1}{l|}{-}                                                                  & 2.16                                                                                          \\ \hline
% \multicolumn{1}{|l|}{CheckSel}                                                   & \multicolumn{1}{l|}{\textcolor{blue}{\textbf{35.76}}}             & \multicolumn{1}{l|}{\textbf{3.6}}                & \multicolumn{1}{l|}{0.4}                                                                & 0.9                                                                                        \\ \hline \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}TracIn-\\ SimSel\end{tabular}}   & \multicolumn{1}{l|}{35.16}              & \multicolumn{1}{l|}{4.62}                & \multicolumn{1}{l|}{-}                                                                  & 2.32                                                                                       \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ SimSel\end{tabular}} & \multicolumn{1}{l|}{\textbf{36.2}}              & \multicolumn{1}{l|}{3.76}                & \multicolumn{1}{l|}{0.4}                                                                & 1.06                                                                                       \\ \hline \hline \hline
% \multicolumn{5}{|l|}{TinyImageNet (10\%, \#CP = 20)}                                                                                                                                                                                                                                                                                                             \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Infl\\ Func\end{tabular}}        & \multicolumn{1}{l|}{11.74}              & \multicolumn{1}{l|}{2.7}                    & \multicolumn{1}{l|}{-}                                                                  & \multicolumn{1}{l|}{-}                                                                                           \\ \hline
% \multicolumn{1}{|l|}{TracIn}                                                     & \multicolumn{1}{l|}{22.84}             & \multicolumn{1}{l|}{12.91}                & \multicolumn{1}{l|}{-}                                                                  & 4.3                                                                                          \\ \hline
% \multicolumn{1}{|l|}{CheckSel}                                                   & \multicolumn{1}{l|}{\textcolor{blue}{\textbf{29.44}}}             & \multicolumn{1}{l|}{12.01}                & \multicolumn{1}{l|}{1.5}                                                                & 1.9                                                                                        \\ \hline \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}TracIn-\\ SimSel\end{tabular}}   & \multicolumn{1}{l|}{23.56}              & \multicolumn{1}{l|}{13.1}                & \multicolumn{1}{l|}{-}                                                                  & 4.49                                                                                       \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ SimSel\end{tabular}} & \multicolumn{1}{l|}{\textbf{29.52}}              & \multicolumn{1}{l|}{12.2}                & \multicolumn{1}{l|}{1.5}                                                                & 2.09                                                                                        \\ \hline
% \end{tabular}
% \end{table}

We also show the normalised residual error (cumulative value function ($I_t$) - estimate) variation with epochs for uniform checkpoint selection, checkpoints with higher loss gap, and CheckSel based selection in Figure \ref{fig:residual}. The normalised residual value for CheckSel is measured by $\frac{|I_{t} (z') - \sum_{i \in S^t}({\alpha_i S_i^t(z_i,z')})|_2}{|I_{t} (z')|_2}$ (notations follow from Section \ref{sec:method}) while for uniform and high loss gap selection, it is measured by $\frac{|I_{t} (z') - \eta \sum_{t'=1}^t \frac{1}{N} \sum_{i \in N}({\nabla l(\theta_{t'},z_i) \nabla l(\theta_{t'}, z')})|_2}{|I_{t} (z')|_2}$ where $t$ refer to the epoch under consideration. We observe that the difference between the residual values vary by a large gap, that gets manifested in the classification performance.

% \begin{table}[]
% \footnotesize
% \caption{Performance Comparison for 10\% subset of CIFAR10}
% \label{tab:addcifar10}
% \begin{tabular}{|p{0.3cm}|c|c|c|p{1.7cm}|c|}
% \hline
% \textbf{\#CP} & \textbf{\begin{tabular}[c]{@{}c@{}}Inf\\ Func\end{tabular}} & \textbf{TracIn} & \textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}} & \textbf{CheckSel} & \textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}} \\ \hline
% 3          & \multirow{4}{*}{59.9}                                                 & \makecell{40.7 \\(2.13T+\\0.3D)}            & \makecell{77.43\\(2.13T+\\0.3D+0.16S)}                                                             & \makecell{78.37\\(2.13T+0.3C+\\0.9D)}           & \makecell{78.63\\\makecell{(2.13T+0.3C+\\0.9D+0.16S)}}                                                               \\ \cline{1-1} \cline{3-6} 
% 5          &                                                                       & \makecell{38.3\\(2.13T+\\0.5D) }            & \makecell{76.76\\(2.13T+\\0.5D+0.16S)}                                                             & \makecell{78.33\\(2.13T+0.3C+\\0.9D) }             &\makecell{79.13\\\makecell{(2.13T+0.3C+\\0.9D+0.16S)}}                                                               \\ \cline{1-1} \cline{3-6} 
% 10         &                                                                       & \makecell{44.13\\(2.13T+\\1D)}           & \makecell{78.63\\(2.13T+\\1D+0.16S)}                                                             & \makecell{79.93\\(2.13T+0.3C+\\0.9D)}            &\makecell{ 79.6\\\makecell{(2.13T+0.3C+\\0.9D+0.16S)}}                                                                \\ \cline{1-1} \cline{3-6} 
% 20         &                                                                       & \makecell{44.73\\(2.13T+\\2D)}           & \makecell{76.9\\(2.13T+\\2D+0.16S)}                                                              & \makecell{79.33\\(2.13T+0.3C+\\0.9D)}             & \makecell{78.7\\\makecell{(2.13T+0.3C+\\0.9D+0.16S)}}                                                                \\ \hline
% \end{tabular}
% \end{table}

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/trac_checksel_acc_cf10_II.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/trac_checksel_acc_cs_cf10_II.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/trac_checksel_acc_cf100_II.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/trac_checksel_acc_cs_cf100_II.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    
    % \begin{subfigure}{0.49\columnwidth}
    % \centering
    % \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/dvtime_cf10.pdf}
    % %\caption{Red light before junction}
    % \end{subfigure}
    \caption{\textbf{Comparison of accuracies between (i) TracIn and CheckSel and (ii) TracIn-Simsel and CheckSel-Simsel across checkpoints for CIFAR10 (\textit{top}) and CIFAR100 (\textit{below}).}}
    \label{fig:varyperf}
\end{figure}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_cf10_tcs.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
    
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_cf10_tcs_ss.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_cf10_tcs_ss_f10.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \caption{\textbf{CIFAR10: Comparison of DV/SS time across checkpoints between (a) TracIn and CheckSel (b) TracIn-Simsel and CheckSel-Simsel for varying fractions of subset.}}
%     \label{fig:varytime1}
% \end{figure}

% \begin{table}[]
% \footnotesize
% \caption{CIFAR10: DV/SS time (hours)comparison}
% \label{tab:cifar10time}
% \centering
% \begin{tabular}{|lllll|}
% \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{Method}}                                    & \multicolumn{4}{c|}{\#CP}                                                                \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                                                           & \multicolumn{1}{l|}{3}    & \multicolumn{1}{l|}{5}    & \multicolumn{1}{l|}{10}   & 20   \\ \hline \hline
% \multicolumn{1}{|l|}{TracIn}                                                     & \multicolumn{1}{l|}{0.3}  & \multicolumn{1}{l|}{0.5}  & \multicolumn{1}{l|}{1}    & 2    \\ \hline
% \multicolumn{1}{|l|}{CheckSel}                                                   & \multicolumn{1}{l|}{0.9}  & \multicolumn{1}{l|}{0.9}  & \multicolumn{1}{l|}{0.9}  & 0.9  \\ \hline \hline
% \multicolumn{5}{|l|}{5\%}                                                                                                                                                   \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}TracIn-\\ Simsel\end{tabular}}   & \multicolumn{1}{l|}{0.45} & \multicolumn{1}{l|}{0.65} & \multicolumn{1}{l|}{1.15} & 2.15 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ Simsel\end{tabular}} & \multicolumn{1}{l|}{1.05} & \multicolumn{1}{l|}{1.05} & \multicolumn{1}{l|}{1.05} & 1.05 \\ \hline
% \multicolumn{5}{|l|}{10\%}                                                                                                                                                  \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}TracIn-\\ Simsel\end{tabular}}   & \multicolumn{1}{l|}{0.46} & \multicolumn{1}{l|}{0.66} & \multicolumn{1}{l|}{1.16} & 2.16 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ Simsel\end{tabular}} & \multicolumn{1}{l|}{1.06} & \multicolumn{1}{l|}{1.06} & \multicolumn{1}{l|}{1.06} & 1.06 \\ \hline
% \end{tabular}
% \end{table}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/trac_checksel_acc_cf100_II.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/trac_checksel_acc_cs_cf100_II.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \caption{\textbf{CIFAR100: Comparison of accuracies between (i) TracIn and CheckSel and (ii) TracIn-Simsel and CheckSel-Simsel across checkpoints via fractions.}}
%     \label{fig:varyperfcf100}
% \end{figure}


% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_cf100_tcs.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
    
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_cf100_tcs_ss_f10.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_cf100_tcs_ss_f15.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \caption{\textbf{CIFAR100: Comparison of DV/SS time across checkpoints between (a) TracIn and CheckSel (b) TracIn-Simsel and CheckSel-Simsel for varying fractions of subset.}}
%     \label{fig:varytime2}
% \end{figure}

% \begin{table}[]
% \footnotesize
% \caption{CIFAR100: DV/SS time (hours)comparison}
% \label{tab:cifar100time}
% \centering
% \begin{tabular}{|lllll|}
% \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{Method}}                                    & \multicolumn{4}{c|}{\#CP}                                                                \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                                                           & \multicolumn{1}{l|}{3}    & \multicolumn{1}{l|}{5}    & \multicolumn{1}{l|}{10}   & 20   \\ \hline \hline
% \multicolumn{1}{|l|}{TracIn}                                                     & \multicolumn{1}{l|}{0.4}  & \multicolumn{1}{l|}{0.54} & \multicolumn{1}{l|}{1.08} & 2.16 \\ \hline
% \multicolumn{1}{|l|}{CheckSel}                                                   & \multicolumn{1}{l|}{0.9}  & \multicolumn{1}{l|}{0.9}  & \multicolumn{1}{l|}{0.9}  & 0.9  \\ \hline \hline
% \multicolumn{5}{|l|}{10\%}                                                                                                                                                  \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}TracIn-\\ Simsel\end{tabular}}   & \multicolumn{1}{l|}{0.57} & \multicolumn{1}{l|}{0.71} & \multicolumn{1}{l|}{1.25} & 2.25 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ Simsel\end{tabular}} & \multicolumn{1}{l|}{1.07} & \multicolumn{1}{l|}{1.07} & \multicolumn{1}{l|}{1.07} & 1.07 \\ \hline
% \multicolumn{5}{|l|}{15\%}                                                                                                                                                  \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}TracIn-\\ Simsel\end{tabular}}   & \multicolumn{1}{l|}{0.59} & \multicolumn{1}{l|}{0.73} & \multicolumn{1}{l|}{1.27} & 2.27 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}CheckSel-\\ Simsel\end{tabular}} & \multicolumn{1}{l|}{1.09} & \multicolumn{1}{l|}{1.09} & \multicolumn{1}{l|}{1.09} & 1.09 \\ \hline
% \end{tabular}
% \end{table}


% \begin{table}[]
% \footnotesize
% \caption{Performance Comparison for 5\% subset of CIFAR10}
% \label{tab:addcifar10_f5}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{\#CP} & \textbf{\begin{tabular}[c]{@{}c@{}}Inf\\ Func\end{tabular}} & \textbf{TracIn} & \textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}} & \textbf{CheckSel} & \textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}} \\ \hline
% 3          & \multirow{4}{*}{35.2}                                                 & \makecell{25.13}            & \makecell{53.6 }                                                             & \makecell{66.9 }             & 65.6                                                               \\ \cline{1-1} \cline{3-6} 
% 5          &                                                                       & \makecell{24.67 }           & \makecell{55.53 }                                                            & \makecell{66.7 }           & 66.6                                                               \\ \cline{1-1} \cline{3-6} 
% 10         &                                                                       & \makecell{26.6  }         & \makecell{56.27 }                                                            & \makecell{67.27  }          & 66.5                                                                \\ \cline{1-1} \cline{3-6} 
% 20         &                                                                       & \makecell{32.23  }         & 57.45                                                              & \makecell{66.47 }            & 67.8                                                                 \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \footnotesize
% \caption{Performance Comparison for 20\% subset of CIFAR10}
% \label{tab:addcifar10_f20}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{\#CP} & \textbf{\begin{tabular}[c]{@{}c@{}}Influence\\ Function\end{tabular}} & \textbf{TracIn} & \textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}} & \textbf{CheckSel} & \textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}} \\ \hline
% 3          & \multirow{4}{*}{83.5}                                                 & 58.53            & 88.57                                                             & 89.37             & 88.67                                                              \\ \cline{1-1} \cline{3-6} 
% 5          &                                                                       & 55.9            & 88.33                                                             & 88.73             & 89.93                                                               \\ \cline{1-1} \cline{3-6} 
% 10         &                                                                       & 60.7           & 88.97                                                             & 88.9            & 88.98                                                                \\ \cline{1-1} \cline{3-6} 
% 20         &                                                                       & 62.76           & 88.95                                                              & 89.1             & 89.23                                                                \\ \hline
% \end{tabular}
% \end{table}



% \begin{table}[]
% \footnotesize
% \caption{Performance Comparison for 10\% subset of CIFAR100}
% \label{tab:addcifar100}
% \begin{tabular}{|p{0.3cm}|p{0.42cm}|c|c|p{1.7cm}|c|}
% \hline
% \textbf{\#CP} & \textbf{\begin{tabular}[c]{@{}c@{}}Inf\\ Func\end{tabular}} & \textbf{TracIn} & \textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}} & \textbf{CheckSel} & \textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}} \\ \hline
% 3          & \multirow{4}{*}{21.82}                                                & \makecell{21.84\\(2.3T+\\0.4D)}          & \makecell{31.4\\(2.3T+\\0.4D+0.16S)}                                                              & \makecell{33.72\\(2.3T+0.4C+\\0.9D)}             & \makecell{32.6\\\makecell{(2.3T+0.4C+\\0.9D+0.16S)}}                                                                \\ \cline{1-1} \cline{3-6} 
% 5          &                                                                       & \makecell{22.04 \\(2.13T+\\0.54D)}           & \makecell{35.44\\(2.3T+\\0.54D+0.16S)}                                                             & \makecell{35.28\\(2.3T+0.4C+\\0.9D) }             & \makecell{36.6\\\makecell{(2.3T+0.4C+\\0.9D+0.16S)}}                                                                \\ \cline{1-1} \cline{3-6} 
% 10         &                                                                       & \makecell{21.48 \\(2.13T+\\1.08D)}           & \makecell{33.96\\(2.3T+\\1.08D+0.16S)}                                                             & \makecell{35.76\\(2.3T+0.4C+\\0.9D)}             & \makecell{35.48\\\makecell{(2.3T+0.4C+\\0.9D+0.16S)}}                                                               \\ \cline{1-1} \cline{3-6} 
% 20         &                                                                       & \makecell{19.44 \\(2.13T+\\2.16D)}           & \makecell{35.16\\(2.3T+\\2.16D+0.16S)}                                                             & \makecell{35.76\\(2.3T+0.4C+\\0.9D) }             & \makecell{36.2\\\makecell{(2.3T+0.4C+\\0.9D+0.16S)}}                                                                \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \footnotesize
% \caption{Performance Comparison for 15\% subset of CIFAR100}
% \label{tab:addcifar100_f15}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{\#CP} & \textbf{\begin{tabular}[c]{@{}c@{}}Inf\\ Func\end{tabular}} & \textbf{TracIn} & \textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}} & \textbf{CheckSel} & \textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}} \\ \hline
% 3          & \multirow{4}{*}{31.4}                                                 & \makecell{31.28}            & \makecell{44.6 }                                                             & \makecell{48.92}             & 48.12                                                                \\ \cline{1-1} \cline{3-6} 
% 5          &                                                                       & \makecell{35.24 }           & \makecell{45.24 }                                                            & \makecell{46.88 }           & 48.2                                                               \\ \cline{1-1} \cline{3-6} 
% 10         &                                                                       & \makecell{32.84 }         & \makecell{45.92 }                                                            & \makecell{47.92  }          & 48.4                                                                 \\ \cline{1-1} \cline{3-6} 
% 20         &                                                                       & \makecell{30.32 }         & 46.64                                                               & \makecell{47.16 }            & 46.82                                                                \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \footnotesize
% \caption{Performance Comparison for 35\% subset of CIFAR100}
% \label{tab:addcifar100_f35}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{\#CP} & \textbf{\begin{tabular}[c]{@{}c@{}}Inf\\ Func\end{tabular}} & \textbf{TracIn} & \textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}} & \textbf{CheckSel} & \textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}} \\ \hline
% 3          & \multirow{4}{*}{53.08}                                                 & 55.8            & 61.8                                                             & 66.04             & 67.44                                                              \\ \cline{1-1} \cline{3-6} 
% 5          &                                                                       & 56.2            & 65.56                                                             &  67.0            & 67.04                                                               \\ \cline{1-1} \cline{3-6} 
% 10         &                                                                       & 54.08           & 63.76                                                             & 66.88            & 67.48                                                                \\ \cline{1-1} \cline{3-6} 
% 20         &                                                                       & 54.12           & 63.24                                                              & 66.8             & 67.04                                                                \\ \hline
% \end{tabular}
% \end{table}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/trac_checksel_acc_tim_II.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/trac_checksel_acc_cs_tim_II.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
    
%     % \begin{subfigure}{0.49\columnwidth}
%     % \centering
%     % \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/dvtime_cf10.pdf}
%     % %\caption{Red light before junction}
%     % \end{subfigure}
%     \caption{\textbf{Tinyimagenet: Comparison of accuracies between (i) TracIn and CheckSel and (ii) TracIn-Simsel and CheckSel-Simsel across checkpoints via fractions.}}
%     \label{fig:varyperftim}
% \end{figure}

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_cf10_tcs.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_cf10_tcs_ss_f10.pdf}
    \end{subfigure}
    % \begin{subfigure}{0.49\columnwidth}
    % \centering
    % \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_cf10_tcs_ss_f10.pdf}
    % %\caption{Red light before junction}
    % \end{subfigure}
    \caption{\textbf{CIFAR10: Comparison of DV/SS time across checkpoints between (a) TracIn and CheckSel (b) TracIn-Simsel and CheckSel-Simsel for 10\% subset.}}
    \label{fig:varytime1}
\end{figure}

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/cs_unif_gap_res_I.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    % \begin{subfigure}{0.49\columnwidth}
    % \centering
    % \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/cs_unif_gap_res_violin.pdf}
    % %\caption{Red light before junction}
    % \end{subfigure}
    \caption{\textbf{Normalised residual values for Uniformly selected, High loss-gap selected and CheckSel selected checkpoints.}}
    \label{fig:residual}
\end{figure}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_tim_tcs.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
    
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_tim_tcs_ss_f10.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/time_tim_tcs_ss_f20.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \caption{\textbf{Tinyimagenet: Comparison of DV/SS time across checkpoints between (a) TracIn and CheckSel (b) TracIn-Simsel and CheckSel-Simsel for varying fractions of subset.}}
%     \label{fig:varytime3}
% \end{figure}

% \begin{table}[]
% \footnotesize
% \caption{Tinyimagenet: DV/SS time (hours)comparison}
% \label{tab:tinyimtime}
% \centering
% \begin{tabular}{|l|ll|}
% \hline
% \multirow{2}{*}{Method}                                    & \multicolumn{2}{c|}{\#CP}        \\ \cline{2-3} 
%                                                           & \multicolumn{1}{l|}{10}   & 20   \\ \hline \hline
% TracIn                                                     & \multicolumn{1}{l|}{2.13} & 4.3  \\ \hline
% CheckSel                                                   & \multicolumn{1}{l|}{1.9}  & 1.9  \\ \hline
% 10\%                                                       & \multicolumn{1}{l|}{}     &      \\ \hline
% \begin{tabular}[c]{@{}l@{}}TracIn-\\ Simsel\end{tabular}   & \multicolumn{1}{l|}{2.32} & 4.49 \\ \hline
% \begin{tabular}[c]{@{}l@{}}CheckSel-\\ Simsel\end{tabular} & \multicolumn{1}{l|}{2.09} & 2.09 \\ \hline
% 20\%                                                       & \multicolumn{1}{l|}{}     &      \\ \hline
% \begin{tabular}[c]{@{}l@{}}TracIn-\\ Simsel\end{tabular}   & \multicolumn{1}{l|}{2.45} & 4.62 \\ \hline
% \begin{tabular}[c]{@{}l@{}}CheckSel-\\ Simsel\end{tabular} & \multicolumn{1}{l|}{2.22} & 2.22 \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \footnotesize
% \caption{Performance Comparison for 10\% subset of Tinyimagenet}
% \label{tab:addtim}
% \begin{tabular}{|p{0.3cm}|p{0.42cm}|c|c|p{1.7cm}|c|}
% \hline
% \textbf{\#CP} & \textbf{\begin{tabular}[c]{@{}c@{}}Inf\\ Func\end{tabular}} & \textbf{TracIn} & \textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}} & \textbf{CheckSel} & \textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}} \\ \hline
% 10          & \multirow{2}{*}{}                                                & \makecell{20.62\\(8.61T+\\D)}           & \makecell{23.46\\(8.61T+\\D+S)}                                                              & \makecell{28.98\\(8.61T+1.5C+\\D)}             & \makecell{29.18\\\makecell{(8.61T+1.5C+\\D+S)}}                                                                \\ \cline{1-1} \cline{3-6} 
% 20          &                                                                       & \makecell{22.84\\(8.61T+\\D)}           & \makecell{23.56\\(8.61T+\\D+S)}                                                             & \makecell{29.44\\(8.61T+1.5C+\\D)}             & \makecell{29.52\\\makecell{(8.61T+1.5C+\\D+S)}}                                                                               \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \footnotesize
% \caption{Performance Comparison for 20\% subset of Tinyimagenet}
% \label{tab:addtim}
% \begin{tabular}{|p{0.3cm}|p{0.42cm}|c|c|p{1.7cm}|c|}
% \hline
% \textbf{\#CP} & \textbf{\begin{tabular}[c]{@{}c@{}}Inf\\ Func\end{tabular}} & \textbf{TracIn} & \textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}} & \textbf{CheckSel} & \textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}} \\ \hline
% 10          & \multirow{2}{*}{19.46}                                                & \makecell{26.18}           & \makecell{26.7}                                                              & \makecell{29.98}             & \makecell{29.92}                                                                \\ \cline{1-1} \cline{3-6} 
% 20          &                                                                       & \makecell{26.16}           & \makecell{26.92}                                                             & \makecell{29.94}             & \makecell{29.88}                                                                               \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \footnotesize
% \caption{Performance Comparison for 30\% subset of Tinyimagenet}
% \label{tab:addtim}
% \begin{tabular}{|p{0.3cm}|p{0.42cm}|c|c|p{1.7cm}|c|}
% \hline
% \textbf{\#CP} & \textbf{\begin{tabular}[c]{@{}c@{}}Inf\\ Func\end{tabular}} & \textbf{TracIn} & \textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}} & \textbf{CheckSel} & \textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}} \\ \hline
% 10          & \multirow{2}{*}{25.7}                                                & \makecell{32.6}           & \makecell{32.74}                                                              & \makecell{34.56}             & \makecell{34.78}                                                                \\ \cline{1-1} \cline{3-6} 
% 20          &                                                                       & \makecell{32.38}           & \makecell{33.98}                                                             & \makecell{34.04}             & \makecell{35.44}                                                                               \\ \hline
% \end{tabular}
% \end{table}



% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/unif_cs_res.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/cs_res.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \caption{\textbf{(a) Normalised residual values for 20 Uniformly selected and Checksel selected checkpoints (b) Zoomed figure for Checksel residual values.}}
%     \label{fig:residual}
% \end{figure}
% \subsection{Addition of instances : $f < |B|$}
% \label{sec:addlower}

% In this section, we show the scenario when the subset size $f$ is less than the number of instances in minibatches ($|\cB|$) obtained through the selected checkpoints using the proposed algorithm. There can be two possibilities of selection; we either take the top instances from the minibatches whose corresponding checkpoints got selected (CheckSel-OnlyB) or we assign scores to all elements and choose the subset from the top scored instances (CheckSel). We show in Figure \ref{tab:addcf10_f2} the performance for 2\% subset of CIFAR10 using $k$ = \{10,20\} ($f$ = 1000, $|\cB| = {1280, 2560}$). We can observe that CheckSel performs better than CheckSel-OnlyB and the other baselines, thus showing that considering all elements while choosing subset is a better alternative.

% This is because, considering only the selected minibatches restricts the diversity as well as the possibility of inclusion of high-scoring elements which may have got eliminated in the form of minibatches while selecting checkpoints. The nearest-neighbour technique aids in assigning scores to all the unattended datapoints, following which the selected subset turns out to be useful for a better performance.

% % \begin{enumerate}
% %     \item Taking only from $\cB$.
% %     \item Taking top elements after finding scores of all elements.
% % \end{enumerate}
% \begin{table}[h]
% \footnotesize
% \caption{Performance Comparison for 2\% subset of CIFAR10}
% \centering
% \label{tab:addcf10_f2}
% \begin{tabular}{|p{0.3cm}|p{0.42cm}|c|c|c|}
% \hline
% \textbf{\#CP} & \textbf{\begin{tabular}[c]{@{}c@{}}Inf\\ Func\end{tabular}} & \textbf{TracIn} & \textbf{\begin{tabular}[c]{@{}c@{}}Checksel-\\ OnlyB\end{tabular}} & \textbf{CheckSel} \\ \hline
% 10          & \multirow{2}{*}{26.7}                                                & \makecell{21.95}           & \makecell{44.67}                                                              & \makecell{44.68}                                                                           \\ \cline{1-1} \cline{3-5} 
% 20          &                                                                       & \makecell{23.65}           & \makecell{44.83}                                                             & \makecell{49.33}                                                                                         \\ \hline
% \end{tabular}
% \end{table}

\subsection{Analysis of selected data}
\label{sec:analyse}

In this section, we intend to demonstrate the usefulness of the selected data through some data maps. We show the fraction of instances selected by TracIn \cite{NEURIPS2020_e6385d39} and CheckSel for CIFAR10 and CIFAR100 (20 superclasses) in Figure \ref{fig:subsetfrac}, that clearly shows the diverse selection of CheckSel, across all classes leading to their better performance.

Inspired by \cite{swayamdipta2020dataset}, we construct data maps to visualise the selected dataset with respect to an underlying model. We use two measures for this purpose - \textit{Confidence} and \textit{Loss}. The intuition is that lower the confidence ($c$) or higher the loss ($l$) of a data point is, harder it is to be classified. We measure the confidence of a datapoint $x_i$ across $T$ epochs as:
\begin{equation}
    c_{x_i} = \frac{1}{T}\sum_{t=1}^T p_{\theta_t} (y_i|x_i)
\end{equation}
where $p_{\theta_t} (y_i|x_i)$ is the probability for $x_i$ to belong to the actual label $y_i$ at epoch $t$. In case of loss, we measure the usual cross-entropy loss for the point $x_i$ across $T$ epochs.

Selecting such harder examples (\textit{low confidence-high loss}) as a part of subset makes the model better thus leading to better performance. We can observe in Figure \ref{fig:datamaps}, the distribution of top 1000 datapoints selected by Checksel from CIFAR10 have comparatively lower confidence and higher loss values, thus denoting the presence of harder examples. We can thus relate this back to their better performance accuracies. The data maps for CIFAR100 and Tinyimagenet are added to Supplementary.

We show a t-SNE diagram in Figure \ref{fig:subsetvis} to visualise the top 1000 datapoints from the subsets obtained using TracIn and CheckSel from CIFAR10. We analyse the t-SNE from three dimensions - class, confidence, loss. We measure the confidence and loss values in 3 levels - High, Medium and Low. We can see that the left-side plots (TracIn) are having a majority of \textit{(bird)} instances (also seen in Figure \ref{fig:subsetfrac}), medium confidence (MC) and medium loss (ML) while the right-side plots (CheckSel) are having a fair mixture of all classes, majority of low confidence (LC) and high loss (HL) points, thus affirming the selection of valuable subsets. Another interesting observation for CheckSel based t-SNE plots are that instances from each of the classes are having a diverse level (\textit{high, medium, low}) of confidence and loss values.

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/propfrac_cf10.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/propfrac_cf100.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    \caption{\textbf{Fraction of top 1000 instances selected by TracIn and CheckSel for CIFAR10 (left) and CIFAR100 (right).}}
    \label{fig:subsetfrac}
\end{figure}


% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/propfrac_cf10.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/propfrac_cf10_uss.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \caption{\textbf{Fraction of instances selected by (a) TracIn and CheckSel (b) TracIn and TracIn-SimSet from CIFAR10}}
%     \label{fig:subsetfrac}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/propfrac_cf100.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/propfrac_cf100_uss.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \caption{\textbf{Fraction of instances selected by (a) TracIn and CheckSel (b) TracIn and TracIn-SimSet from CIFAR100}}
%     \label{fig:subsetfraccf100}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/plot_tracin.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     %\caption{\textbf{Performance on CIFAR10}}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/plot_checksel.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \caption{\textbf{t-SNE plot of selected datapoints using (a) TracIn and (b) CheckSel}}
%     \label{fig:subsetvis}
% \end{figure}
\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/confi-cifar10.pdf}
    \end{subfigure}
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/loss-cifar10.pdf}
    \end{subfigure}
    \caption{\textbf{CIFAR10: Distribution of confidence and loss values of datapoints selected by TracIn and CheckSel.}}
    \label{fig:datamaps}
\end{figure}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/confi-cifar100.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/loss-cifar100.pdf}
%     \end{subfigure}
%     \caption{\textbf{Data Maps for CIFAR100}}
%     \label{fig:datamaps_cf100}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/confi-tim.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/loss-tim.pdf}
%     \end{subfigure}
%     \caption{\textbf{Data Maps for Tinyimagenet}}
%     \label{fig:datamaps_tim}
% \end{figure}


\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/tracin_class_tsne_I.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    %\caption{\textbf{Performance on CIFAR10}}
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/checksel_class_tsne_I.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/tracin_conf_tsne_I.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    %\caption{\textbf{Performance on CIFAR10}}
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/checksel_conf_tsne_I.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/tracin_loss_tsne_I.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    %\caption{\textbf{Performance on CIFAR10}}
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/checksel_loss_tsne_I.pdf}
    %\caption{Red light before junction}
    \end{subfigure}
    \caption{\textbf{t-SNE embeddings of selected datapoints using TracIn (left) and CheckSel (right) shown based on classes (top) and confidence (middle) and loss (below) values.}}
    \label{fig:subsetvis}
\end{figure}



% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/tracin_class_tsne.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     %\caption{\textbf{Performance on CIFAR10}}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/checksel_class_tsne.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
    
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/tracin_confloss_tsne.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     %\caption{\textbf{Performance on CIFAR10}}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/checksel_confloss_tsne.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \caption{\textbf{t-SNE plot of selected datapoints using TracIn (left) and CheckSel (right) based on classes (top) and confidence-loss values (below)}}
%     \label{fig:subsetvis}
% \end{figure}



% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/confidence-cifar100.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/loss-cifar100.pdf}
%     \end{subfigure}
%     \caption{\textbf{Data Maps for CIFAR100}}
%     \label{fig:datamaps_cf100}
% \end{figure}

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/conf_freq_tracin.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/conf_freq_checksel.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/loss_freq_tracin.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/loss_freq_checksel.pdf}
%     \end{subfigure}
%     \caption{\textbf{Data Maps for CIFAR10}}
%     \label{fig:datamaps}
% \end{figure*}

% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/conf_freq_tracin_cf100.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/conf_freq_checksel_cf100.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/loss_freq_tracin_cf100.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/loss_freq_checksel_cf100.pdf}
%     \end{subfigure}
%     \caption{\textbf{Data Maps for CIFAR100}}
%     \label{fig:datamaps_cf100}
% \end{figure*}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/confpoints.pdf}
%     \end{subfigure}
%     \begin{subfigure}{0.49\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3.5cm]{latex/figs/losspoints.pdf}
%     \end{subfigure}
%     \caption{\textbf{Data Maps}}
%     \label{fig:datamaps}
% \end{figure}


\subsection{Domain adaptation}
\label{sec:domadapt}
In this section, our aim is to find a subset from the target domain without including it during the source domain training procedure. We use the source dataset for training and selecting checkpoints that will be used to find the subset on target domain. We use the feature extraction model obtained while training the source dataset to compute the embeddings of both source and target domain, that will aid in finding the nearest neighbour for the target domain examples, from the source domain set. Following this in the data selection phase, we can obtain the scores of each instance in target domain. 
% Additionally, we also test the proposed method by including the target domain validation set in the value function, terming it as CheckSel-Target.

We use the Office-Home dataset \cite{venkateswara2017deep} containing 4 domains - Art, Clipart, Product, Real-World, each with 65 categories and ResNet-50 model with fine-tuning. The source ($D_s$) and target ($D_t$) datasets will be mapped from one domain to another. Both $D_s$ and  $D_t$ are divided into training and validation counterparts ($D_{st}$ , $D_{sv}$ and $D_{tt}$ , $D_{tv}$) respectively. We train on $D_{st}$ keeping $D_{sv}$ and $D_{tv}$ as the validation set interchangeably, for computing the value function terming them as CheckSel-Source-Val and CheckSel-Target-Val respectively, following which we select checkpoints using Algorithm \ref{algo:onlineomp}.

Next, we compute scores of each element $e \in D_{tt}$ by finding nearest neighbour from $D_{st}$ using the trained feature extractor. Following this, we acquire the subsets of the target domain and train them with No Domain Adaptation (NDA). We call the method ''CheckSel-Source-Val-NDA'' and ''CheckSel-Target-Val-NDA'' based on the validation set used in the value function. We show our results in Table \ref{tab:daofficehome} with \textit{Art, ClipArt, Product, RealWorld} as the source domain respectively and the other three as the target domain. We train on a subset of 20\% data from target domain using 20 selected checkpoints obtained while training on the source domain and test on the target domain too. We also perform domain adaptation (DA) training following \cite{Xu_2019_ICCV}\footnote{https://github.com/jihanyang/AFN} taking source and target subsets obtained from CheckSel-Source-Val, terming it as CheckSel-Source-Val-DA. This configuration is similar to CheckSel-Source-Val with an additional objective of reducing the loss between the embeddings of the source subset and target subset. Figure \ref{fig:dataval_da} illustrates the same graphically.

\begin{figure}[h!]
    %\centering
    %\begin{subfigure}{0.48\columnwidth}
    \centering
    \includegraphics[width=0.85\columnwidth,height=5cm]{latex/figs/Domain adaptation.pdf}
    %\end{subfigure}
    \caption{\textbf{Domain adaptation data valuation on target domain}}
    \label{fig:dataval_da}
\end{figure}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.9\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=4.5cm]{latex/figs/Domain adaptation.pdf}
%     %\caption{Red light before junction}
%     \end{subfigure}
%     \caption{\textbf{Domain adaptation data valuation on target domain}}
%     \label{fig:dataval_da}
% \end{figure}

We can observe that CheckSel-Target performs the best across most source to target domains while CheckSel-Source-DA is the next best followed by CheckSel-Source. It can be observed that TracIn has a significantly lower accuracy compared to the variants of our proposed methods, thus denoting the effectiveness of the algorithm even in absence of target domain during training. We also show some anecdotal examples in Figure \ref{fig:anecdotal} where we can see for Product $->$ Art domain, the top samples selected by CheckSel are far more diverse (\textit{laptop, flower,speaker, fan}) than by TracIn (\textit{laptop, mouse}), thus having significantly high performance.

\begin{table}[h]
\footnotesize
\centering
\caption{\textbf{Performance Comparison on Office-Home}}
\label{tab:daofficehome}
\begin{tabular}{|p{2cm}|l|l|l|l|}
\hline
\textbf{Source-\textgreater{}Target}  & \textbf{TracIn} &\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}l@{}}CheckSel\\Source-Val\\NDA\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}l@{}}CheckSel\\Target-Val\\NDA\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}l@{}}CheckSel\\Source-Val\\DA\end{tabular}}} \\ \hline
Art-\textgreater{}ClipArt    & 31.4   & 47.99 & \textbf{54.97} & 52.48   \\ \hline
Art-\textgreater{}Product    & 33.95  & 70.11 & \textbf{75.23} & 72.2 \\ \hline
Art-\textgreater{}Real World & 34.63  & 67.49 & 71.04 & \textbf{71.63} \\ \hline
Art-\textgreater{}Art & 36.34   & 52.26 & -  & - \\ \hline
\hline
ClipArt-\textgreater{}Art    & 36.34   & 51.61 & \textbf{53.98} & 51.18 \\ \hline
ClipArt-\textgreater{}Product    & 39.76  & 69.18 & \textbf{75.74} & 69.43 \\ \hline
ClipArt-\textgreater{}Real World & 34.87  & 65.48 & \textbf{74.05} & 64.54 \\ \hline 
ClipArt-\textgreater{}ClipArt & 33.09  & 52.3 & -  & - \\ \hline \hline
Product-\textgreater{}Art    & 34.62   & 54.4 & \textbf{56.55} & 56.13 \\ \hline
Product-\textgreater{}ClipArt    & 30.85  & 57.32 & 57.21 & \textbf{59.57}\\ \hline
Product-\textgreater{}Real World & 36.28  & 69.03 & \textbf{73.04} & 70.8 \\ \hline
Product-\textgreater{}Product & 35.81  & 65.59 & -  & -\\ \hline  \hline
Real World-\textgreater{}Art    & 33.76   & 50.75 & \textbf{56.56}  & 56.34 \\ \hline
Real World-\textgreater{}ClipArt    & 29.9  & 48.46 & 50.47 & \textbf{51.3} \\ \hline
Real World-\textgreater{}Product & 33.25  & 64.41 & \textbf{70.97} & 68.25  \\ \hline
Real World-\textgreater{}Real World  & 35.22   & 60.4 & -   & - \\ \hline
\end{tabular}
\end{table}

% \begin{table*}[h]
% \footnotesize
% \centering
% \caption{\textbf{Performance Comparison on Office-Home}}
% \label{tab:daofficehome}
% \begin{tabular}{|p{2cm}|l|l|l|l|l|}
% \hline
% \textbf{Source-\textgreater{}Target}  & \textbf{TracIn} &\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Checksel\\Source\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Checksel\\Targ\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Checksel\\Source-DA\end{tabular}}} & \textbf{CheckSel-Targ-DA} \\ \hline
% Art-\textgreater{}ClipArt    & 31.4   & \textcolor{blue}{47.99} & \textcolor{blue}{54.97} & 52.48 & 60.16   \\ \hline
% Art-\textgreater{}Product    & 33.95  & \textcolor{blue}{70.11} & \textcolor{blue}{75.23} & 72.2 & 77.79 \\ \hline
% Art-\textgreater{}Real World & 34.63  & \textcolor{blue}{67.49} & \textcolor{blue}{71.04} & 71.63 & 73.99      \\ \hline
% Art-\textgreater{}Art & 36.34   & \textcolor{blue}{52.26} & -  & - & -       \\ \hline
% \hline
% ClipArt-\textgreater{}Art    & 36.34   & \textcolor{blue}{51.61} & \textcolor{blue}{53.98} & 51.18 & 57.84  \\ \hline
% ClipArt-\textgreater{}Product    & 39.76  & \textcolor{blue}{69.18} & \textcolor{blue}{75.74} & 69.43 & 77.02   \\ \hline
% ClipArt-\textgreater{}Real World & 34.87  & \textcolor{blue}{65.48} & \textcolor{blue}{74.05} & 64.54 & 75.05       \\ \hline 
% ClipArt-\textgreater{}ClipArt & 33.09  & \textcolor{blue}{52.3} & -  & - & -      \\ \hline \hline
% Product-\textgreater{}Art    & 34.62   & \textcolor{blue}{54.4} & \textcolor{blue}{56.55} & 56.13 & 59.47  \\ \hline
% Product-\textgreater{}ClipArt    & 30.85  &\textcolor{blue}{57.32} & \textcolor{blue}{57.21} & 59.57 & 61.58   \\ \hline
% Product-\textgreater{}Real World & 36.28  & \textcolor{blue}{69.03} & \textcolor{blue}{73.04} & 70.8 & 74.94      \\ \hline
% Product-\textgreater{}Product & 35.81  & \textcolor{blue}{65.59} & -  & - & -      \\ \hline \hline
% Real World-\textgreater{}Art    & 33.76   & \textcolor{blue}{64.94} & \textcolor{blue}{56.56}  & 56.34 & 61.93   \\ \hline
% Real World-\textgreater{}ClipArt    & 29.9  & \textcolor{blue}{48.46} & \textcolor{blue}{50.47} & 51.3 & 55.05   \\ \hline
% Real World-\textgreater{}Product & 33.25  & \textcolor{blue}{64.41} & \textcolor{blue}{70.97} & 68.25 & 74.21       \\ \hline
% Real World-\textgreater{}Real World  & 35.22   & \textcolor{blue}{60.4} & -   & - & -     \\ \hline
% \end{tabular}
% \end{table*}


\begin{figure}[h!]
    \centering
        \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/unif_art/1.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/unif_art/2.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/unif_art/3.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/unif_art/4.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/unif_art/5.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/unif_art/6.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/unif_art/7.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/unif_art/8.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/unif_art/9.jpg}
    \end{subfigure}

    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/cs_art/1.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/cs_art/2.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/cs_art/3.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/cs_art/4.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/cs_art/5.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/cs_art/6.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/cs_art/7.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/cs_art/8.jpg}
    \end{subfigure}
    \begin{subfigure}{0.1\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=1cm]{latex/figs/cs_art/10.jpg}
    \end{subfigure}
    \caption{\textbf{Top selected examples from Art domain for Product $->$ Art experiment using TracIn (above) \& CheckSel (below)}}
    \label{fig:anecdotal}
\end{figure}
% \begin{table}[h]
% \footnotesize
% \centering
% \caption{\textbf{Performance Comparison on Office-Home}}
% \label{tab:daofficehome}
% \begin{tabular}{|p{2cm}|l|l|l|}
% \hline
% \textbf{Source-\textgreater{}Target}  & \textbf{TracIn} & \textbf{CheckSel-Source} & \textbf{CheckSel-Targ} \\ \hline
% Art-\textgreater{}ClipArt    & 31.4   & \textcolor{blue}{47.99} & \textcolor{blue}{54.97}    \\ \hline
% Art-\textgreater{}Product    & 33.95  & \textcolor{blue}{70.11} & \textcolor{blue}{75.23}   \\ \hline
% Art-\textgreater{}Real World & 34.63  & \textcolor{blue}{67.49} & \textcolor{blue}{71.04}        \\ \hline
% Art-\textgreater{}Art & 36.34   & \textcolor{blue}{52.26} & -         \\ \hline
% \hline
% ClipArt-\textgreater{}Art    & 36.34   & \textcolor{blue}{51.61} & \textcolor{blue}{53.98}  \\ \hline
% ClipArt-\textgreater{}Product    & 39.76  & \textcolor{blue}{69.18} & \textcolor{blue}{75.74}   \\ \hline
% ClipArt-\textgreater{}Real World & 34.87  & \textcolor{blue}{65.48} & \textcolor{blue}{74.05}       \\ \hline 
% ClipArt-\textgreater{}ClipArt & 33.09  & \textcolor{blue}{52.3} & -       \\ \hline \hline
% Product-\textgreater{}Art    & 34.62   & \textcolor{blue}{54.4} & \textcolor{blue}{56.55}  \\ \hline
% Product-\textgreater{}ClipArt    & 30.85  &\textcolor{blue}{57.32} & \textcolor{blue}{57.21}   \\ \hline
% Product-\textgreater{}Real World & 36.28  & \textcolor{blue}{69.03} & \textcolor{blue}{73.04}       \\ \hline
% Product-\textgreater{}Product & 35.81  & \textcolor{blue}{65.59} & -       \\ \hline \hline
% Real World-\textgreater{}Art    & 33.76   & \textcolor{blue}{64.94} & \textcolor{blue}{55.91}    \\ \hline
% Real World-\textgreater{}ClipArt    & 29.9  & \textcolor{blue}{48.46} & \textcolor{blue}{50.47}   \\ \hline
% Real World-\textgreater{}Product & 33.25  & \textcolor{blue}{64.41} & \textcolor{blue}{70.97}        \\ \hline
% Real World-\textgreater{}Real World  & 35.22   & \textcolor{blue}{60.4} & -       \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \centering
% \caption{\textbf{Performance Comparison on Office-Home}}
% \label{tab:officehome}
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Domain}  & \textbf{TracIn} & \textbf{CheckSel} \\ \hline
% Art    & 36.34   & \textcolor{blue}{52.26}   \\ \hline
% ClipArt    & 33.09  & \textcolor{blue}{52.3}    \\ \hline
% Product & 35.81  & \textcolor{blue}{65.59}         \\ \hline
% Real World    & 35.22   & \textcolor{blue}{60.4}    \\ \hline
% \end{tabular}
% \end{table}
% \begin{table*}
% \scriptsize
% \centering
% \caption{Performance comparison on CIFAR10}
% \label{tab:addcifar10}
% \begin{tabular}{|l|l|c|l|l|l|c|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Fraction}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Influence\\ Functions\end{tabular}}}} & \multicolumn{4}{c|}{\textbf{k = 3}}                                                                                                                                                                                                                     & \multicolumn{4}{c|}{\textbf{k = 5}}                                                                                                                                                                                                                     \\ \cline{3-10} 
% \multicolumn{1}{|c|}{}                                   & \multicolumn{1}{c|}{}                                                                                        & \textbf{TracIn}            & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}}} & \multicolumn{1}{c|}{\textbf{CheckSel}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}}} & \textbf{TracIn}            & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}TracIn-\\ SimSet\end{tabular}}} & \multicolumn{1}{c|}{\textbf{CheckSel}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}CheckSel-\\ SimSet\end{tabular}}} \\ \hline
% \multirow{3}{*}{10\%}                                    & 59.9 \multirow{3}{*}{}                                                                                            & \multicolumn{1}{l|}{40.17} & 77.43                                                                                  & 78.37                                  & \textbf{78.63}                                                                                    & \multicolumn{1}{l|}{38.3}  & 76.76                                                                                  & 78.33                                  & \textbf{79.13}                                                                                    \\ \cline{3-10} 
%                                                          &                                                                                                              & \multicolumn{4}{c|}{\textbf{k = 10}}                                                                                                                                                                                                                    & \multicolumn{4}{c|}{\textbf{k = 20}}                                                                                                                                                                                                                    \\ \cline{3-10} 
%                                                          &                                                                                                              & \multicolumn{1}{l|}{44.13} & 78.63                                                                                  & \textbf{79.93}                                  & 79.6                                                                                     & \multicolumn{1}{l|}{44.73} & 76.9                                                                                   & \textbf{79.33}                                  & 78.7                                                                                     \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table}[h]
% \caption{Performance comparison between \textit{UnifSelect} and \textit{CheckSelect - Technique 2} for 5\% subset}
% \centering
% \begin{tabular}{ |c|c|c| }
%  \hline
%   \textbf{Checkpoints(k)} & \textbf{UnifSelect} & \textbf{CheckSelect} \\
%   \hline
%  3 & 28.25 & 64.4 \\ 
%  \hline
%  5 & 25.25 & 64.4\\ 
%  \hline
%  10 & 27.05 & 67.5\\
%  \hline
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \caption{Performance comparison between \textit{UnifSelect} and \textit{CheckSelect - Technique 1} for 1\% subset}
% \centering
% \begin{tabular}{ |c|c|c| }
%  \hline
%   \textbf{Checkpoints(k)} & \textbf{UnifSelect} & \textbf{CheckSelect} \\
%   \hline
%  10 & 19.35 & 34.4 \\ 
%  \hline
%  20 & 19.5 & 34.55\\ 
%  \hline
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \caption{Performance comparison between \textit{UnifSelect} and \textit{CheckSelect - Technique 1} for 2\% subset}
% \centering
% \begin{tabular}{ |c|c|c| }
%  \hline
%   \textbf{Checkpoints(k)} & \textbf{UnifSelect} & \textbf{CheckSelect} \\
%   \hline
%  10 & 21.95 & 43.25\\ 
%  \hline
% 20 & 23.65 & 43.15\\ 
%  \hline
% \end{tabular}
% \end{table}

==> method.tex <==

\newcommand{\tr}[1]{\textcolor{red}{#1}}

\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\RR}{\mathbb{R}}
\newtheorem{theorem}{Theorem}
% \title{Formulation Subset TracIn}
% \author{}
% \date{}
\section{Online Checkpoint Selection}

%Subset selection using data valuation is an efficient technique for filtering out the important training points necessary for explaining the predictions of a deep neural network model. 
In this section, we introduce the proposed data valuation method \textit{\ourmethod} -- a two-phase selection method using the training run of a gradient descent algorithm. The first phase selects informative checkpoints from the training algorithm, and  the second phase computes the value each datapoint. 
%Our novelty lies in the checkpoint selection obtaining which, we proceed to the next phase, datapoint selection, that is adapted from \cite{NEURIPS2020_e6385d39}.

\subsection{Data valuation using training trajectories}

We briefly review the TracIn \cite{NEURIPS2020_e6385d39} method.
Let $\mathcal{Z} = \{ z_i = (x_i , y_i)| i = 1,2,..,N\}$ be the training dataset for a supervised learning task with features $x_i \in \mathcal{X}$ and labels $y_i \in \mathcal{Y}$. Also, let $\mathcal{Z'} = \{ z'_j = (x'_j , y'_j)| j = 1,2,..,M\}$ be the valuation/test dataset which is used for assigning values/scores to a training datapoint $z\in \mathcal{Z}$. Additionally, let $\theta_1,...,\theta_T$ be a sequence of parameters generated by training with a given deep learning model on training dataset $\cZ$ using a mini-batch SGD-like algorithm.
TracIn \cite{NEURIPS2020_e6385d39} defines the scores for each training datapoint $z$, given a valuation datapoint $z'$ as the first order approximation for decrease in 
\begin{equation}
    l(\theta_{t+1},z') - l(\theta_t,z') =  \nabla l(\theta_t, z').(\theta_{t+1} - \theta_t)
\label{eqn:ap1}
\end{equation}
% $l(\theta_{t+1},z') - l(\theta_t,z') =  \nabla l(\theta_t, z').(\theta_{t+1} - \theta_t)$ 
where $l(\theta_t,z')$ is the loss(value function) on $z'$ using end-epoch model parameter $\theta_t$. The influence/score of any training point $z$ on the test set $\mathcal{Z'}$, being termed as \textit{TracIn}$(z,\mathcal{Z}')$ \cite{NEURIPS2020_e6385d39} uses parameters from uniformly selected end-epoch checkpoints $t = 1,2,..,T$ of a trained model and is defined as:
\begin{equation}
    TracIn(z,\mathcal{Z}') = \sum_{t=1}^T \nabla_{\theta_t} l (\theta_t, z).\nabla_{\theta_t} l (\theta_t, \mathcal{Z}')
\label{eq:tracin}
\end{equation}

We argue that the uniformly selected end-epoch checkpoints might not be a good measure for the above mentioned approximation since it does not consider the intermediate checkpoints while approximating $(\theta_{t+1} - \theta_t)$ (from first order) to $\nabla_{\theta_t} l (\theta_t, z)$, that shall be necessary in a mini-batch update setup. Hence, we propose a better approximation over the uniformly selected checkpoints.

\subsection{Proposed Approximation}
From first-order approximation of the value function (in this case test-set loss), we know
\begin{equation}
    l(\theta_{t+1},z') - l(\theta_t,z') =  \nabla l(\theta_t, z').(\theta_{t+1} - \theta_t)
\label{eqn:ap1}
\end{equation}

Assuming $\theta_{t}^0 = \theta_t$ and $\theta_{t}^O = \theta_{t+1}$ (total $O$ minibatches in epoch $t$), we can rewrite Equation \ref{eqn:ap1} as:

\begin{equation}
    \sum_{i=1}^O l(\theta_{t}^i,z') - l(\theta_{t}^{i-1},z') =  \sum_{i=1}^O (\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z')
\label{eqn:ap2}
\end{equation}

%where i denotes the batch number.

In this context, we adopt the 2nd order approximation where $(\nabla l(\theta_{t}^{i-1}, z'))^2$ is an approximate form of $\nabla^2 l(\theta_{t}^{i-1}, z')$. So we rewrite Equation \ref{eqn:ap2} as:

\begin{align}
    & \Vec{\triangle}_{t}(z') =
    \sum_{i=1}^O l(\theta_{t}^i,z') - l(\theta_{t}^{i-1},z') = \nonumber \\ & \sum_{i=1}^O (\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z') \nonumber \\ & + 0.5*((\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z'))^2
\label{eqn:ap2c}
\end{align}
where $\Vec{\triangle}_{t}(z')$ denotes change in test set loss over minibatches for epoch $t$.
% Let us call L.H.S of Eqn \ref{eqn:ap2c} as $\Vec{\triangle}_{t}(z')$ denoting change in test set loss over minibatches for epoch $t$:

% \begin{equation}
%     \Vec{\triangle}_{t} (z') = 
%     \sum_{i=1}^O l(\theta_{t}^i,z') - l(\theta_{t}^{i-1},z')
% \label{eqn:ap3}
% \end{equation}

%Let $\theta_{t}^{i}$ denote the SGD update.
Using the mini-batch weight update $\theta_{t}^{i} = \theta_{t}^{i-1} - \eta \nabla l(\theta_{t}^{i-1},z_i)$ , we can rewrite Equation \ref{eqn:ap2c} as: 

% \begin{equation}
%      \Vec{\triangle}_{t} (z') \approx \sum_{i=1}^O (\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z') + \nonumber \\ 0.5*((\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z'))^2
% \label{eqn:ap5}
% \end{equation}

% Using the update in Equation \ref{eqn:ap5}, we get:
\begin{align}
    \Vec{\triangle}_{t} (z') \approx -\eta \sum_{i=1}^O \nabla l(\theta_{t}^{i-1},z_i)^T \nabla l(\theta_{t}^{i-1}, z') \nonumber \\  + 0.5*(\nabla l(\theta_{t}^{i-1},z_i)^T \nabla l(\theta_{t}^{i-1}, z'))^2 \nonumber \\ \approx -\eta \sum_{i=1}^O \Vec{\mathcal{C}}_{i}^t(z_{i},z')
\label{eqn:ap6}
\end{align}

where $\Vec{\mathcal{C}}^{t}(z_{i},z')$ denotes the contribution of $z_{i}$ on $z'$ at epoch $t$ or similarity in gradients. $\Vec{\triangle}_{t} (z')$ is of the size $|$test set size$| \times$ 1 , while $\Vec{\mathcal{C}}^{t}(z,z')$ is of the size $|$test set size$| \times$ O

Mapping it to Orthogonal Matching Pursuit (OMP) problem where we want to form a set S containing $k$ out of $O$ checkpoints, the objective function comes to:

\begin{equation}
    \min ||\sum_{i \in S_{t}}({\alpha_i \Vec{\mathcal{C}}_{i}^t(z_i,z')}) - \Vec{\triangle}_{t}(z')||_2 \hspace{3mm} s.t. ||\alpha||_0 \leq k
\end{equation}

However, we propose to perform the selection in an online manner across epochs during the training. Hence, we propose an online version of OMP for selection of $k$ checkpoints.

\subsection{Phase 1: OMP based checkpoint selection}
\label{sec:oomp}

Consider the cumulative $\Delta_t$ vector that denotes the cumulative change in loss across epochs, 
$$I_t = \sum_{j=1}^t \Delta_j\ \ \forall t=1,...,T$$
% Also, let $C^t_i \in \RR^M \forall i\in \{1,...,O\}$, where $O$ is the number of number of batches in each epoch. 

In the online setting, at time $t$ we want to approximate:
$$ I_t \approx \sum_{j\in \cR^t} \alpha_j S^t_j $$ where, $\cS$ is the set having the gradient similarities of selected minibatches over time ad $\cR$ is the set of selected checkpoint/minibatch indices. So $\cS$ is of the size $|$test set size$| \times$ k. So, from Equation \ref{eqn:ap6}, we can rewrite the above approximation as:\\
\begin{align}
\label{eq:finalapp}
     I_t \approx \eta \sum_{j\in \cR^t} \alpha_j [\nabla l(\theta_{t}^{j-1},z_j)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j)^T \nabla l(\theta_{t}^{j-1}, z'))^2] 
\end{align}



The idea is to keep track of the selected checkpoints over time, and replace them with incoming checkpoints, based on their projections with the residual, which is the difference between the obtained estimate ($\xi = \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i$) and the ground truth ($I^t$ in this case). The detailed description is provided in Algorithm \ref{algo:onlineomp} and \ref{algo:replace}. 

% \textcolor{red}{Note for thought: Tweaking Online OMP algorithm to approximate the extrapolation during data valuation in Phase 2}
% Having obtained the set of checkpoints $S$, we compute the scores for each training point $z_i$ using the approximated estimate $\sum_{j\in \cS} \alpha_j S_j$.

 \begin{minipage}{0.46\textwidth}
 \begin{algorithm}[H]
 \caption{: Online OMP}
 \label{algo:onlineomp}
 %\scriptsize
 %\label{algo:onlineomp}
 \begin{algorithmic}[1]
\State{\textbf{Input}:} $k$: Total number of checkpoints to be selected\\
$I$: Cumulative change in loss;
$C$: Gradient similarity

 \State \textbf{Initialize:}
 Set of selected components from C: $\cS$ = $\phi$\\
 Set of weights for the selected components: $\alpha = zero_{|S|}$ \\
 Estimate $\xi = \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i$, initially 0
%  Let the estimate $\xi = 0$ be the running estimate defined as $\sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i $ where $\alpha_i\in \alpha$ and $S_i\in \cS$
 
 \For{t = 1,...,T}
 \State \textbf{Input:} $I_t, C_i^t , \forall i\in\{1,...,O\} , ||C_i||_2 = 1 $
 \State{\textbf{Process}:}
 \State  Update $\alpha : argmin_\alpha \|\sum_{i \in |S|}(\alpha_i S_i) - I^t||_2$
 \State Update $\xi : \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i$
% \State $est = \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i $
% \State $res = I^t - est$
 \For{each batch $i \in O$:}
 \State ** Replacing selected checkpoints **
 \If{$|\cS| = k$}
 \State $\cS , \alpha, \xi$ = \textbf{Replace($I^t , \xi, \cS, \alpha , C_i^t$)}
 \Else
 \State ** Add the checkpoints sequentially **
 \State  $\cS \longleftarrow \cS \cup \{C_i^t\}$
 \State  Update $\alpha$ ; Update $\xi$
 \EndIf
 \EndFor
 \EndFor
 \State \textbf{Output}:Final set of selected checkpoints , $\cS$
 \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
 %\scriptsize
 \caption{: \textbf{Replace ($I^t , \xi, \cS, \alpha , C_i^t$)}}
 \label{algo:replace}
 \begin{algorithmic}[1]
\State  $\rho = I^t - \xi$ \*//Residual
 \State $maxproj = -\infty$ \*// best projection from existing set
 \State $ind = \phi$ \* /index of the best projection from existing set
 \For{each index $j$ in $\cS$:}
 %\State If{$|\cS| = k$}
 \State  $n\rho = \rho + \alpha_j*S_j$ \*// new residual on including $S_j$
 \State  $n\varrho = C_i^t . n\rho$  \*//projection of $C_i^t$ , incoming gradient
 \State  $\varrho = S_j . n\rho$  \*//projection of $S_j$, existing gradient
  \If{$n\varrho > \varrho$ and $n\varrho>maxproj$}
 \State maxproj $\longleftarrow$  $\varrho$
 \State $ind = j$
 \EndIf
 \EndFor
 \If{$ind \neq \phi$}
%  \State $S_{ind} \longleftarrow C_i^t$  \*//Replace $S_{ind}$ with $C_i^t$ which has higher projection than the best in set S: $S_{ind}$
 \State $S_{ind} \longleftarrow C_i^t$  \*//Replace the best existing projection in $S$ with the new projection
  \State Update $\alpha$ ; Update $\xi$
 \EndIf \\
 return $\cS, \alpha, \xi$
 \end{algorithmic}
\end{algorithm}
% \begin{algorithm}[H]
%  \scriptsize
%  \caption{: \textbf{Replace ($I^t , \xi, \cS, \alpha , C_i^t$)}}
%  \label{algo:replace}
%  \begin{algorithmic}[1]
% \State  $\rho = I^t - \xi$ \*//Residual
%  \State $maxproj = -\infty$ \*// best projection from existing set
%  \State $ind = \phi$ \* /index of the best projection from existing set
%  \For{each index $j$ in $\cS$:}
%  %\State If{$|\cS| = k$}
%  \State  $n\rho = \rho + \alpha_j*S_j$ \*// new residual on including $S_j$
%  \State  $n\varrho = C_i^t . n\rho$  \*//projection of $C_i^t$ , incoming gradient
%  \State  $\varrho = S_j . n\rho$  \*//projection of $S_j$, existing gradient
%   \If{$n\varrho > \varrho$ and $n\varrho>maxproj$}
%  \State maxproj $\longleftarrow$  $\varrho$
%  \State $ind = j$
%  \EndIf
%  \EndFor
%  \If{$ind \neq \phi$}
% %  \State $S_{ind} \longleftarrow C_i^t$  \*//Replace $S_{ind}$ with $C_i^t$ which has higher projection than the best in set S: $S_{ind}$
%  \State $S_{ind} \longleftarrow C_i^t$  \*//Replace the best existing projection in $S$ with the new projection
%   \State Update $\alpha$ ; Update $\xi$
%  \EndIf \\
%  return $\cS, \alpha, \xi$
%  \end{algorithmic}
% \end{algorithm}
\end{minipage}
\subsection{Phase 2: Data valuation using selected checkpoints}

The final approximation is demonstrated in Equation \ref{eq:finalapp} where $\cS$ contains the gradient similarity values w.r.t selected checkpoints. We can also rewrite Equation \ref{eq:finalapp} as:
\begin{align}
\label{eq:finalapp2}
     I_t \approx \eta \sum_{j\in \cR^t} \frac{1}{|\cB_j|} \sum_{i\in \cB_j} \alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2] 
\end{align}

where $\cB_j$ is the mini-batch associated with the selected checkpoint j $\in \cR$ and $z_j^i \in \cB_j$ is the i-th datapoint in $\cB_j$.
We associate the similarity in gradients (Equation \ref{eq:finalapp2}) to score/data value of the training points $\in \cB$ since that denotes the impact of the training point on the test set performance. We define the score in Equation \ref{eq:score}.

\begin{align}
\label{eq:score}
Value(z_j^i \in \cB_j) = \frac{1}{|\cB_j|} \sum_{z' \in \cZ'} (\alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2])
\end{align}

In order to select a subset of a given cardinality $f$, we can follow some techniques given below: 
\begin{enumerate}
    \item If $f < |\cB|$, where $|\cB|$ = $\sum_{j \in \cR} |\cB_j|$, we can take the top $f$ elements from $\cB$ in order of their scores obtained from Equation \ref{eq:score}.
    %\item Otherwise, we can take all the elements from $\cB$ and choose $f-|\cB|$ elements randomly from $\cZ \setminus \cB$.
    \item Otherwise, for $f > |B|$ we % form clusters with the selected elements $\in \cB$ (using feature values from trained model) and 
    find the nearest neighbouring point $n \in \cB$ (using some form of feature similarity) for each element $e$ in $\cZ \setminus \cB$. Following that, we can
    % either assign \textit{Value(e)} = \textit{Value(n)} , or 
    compute \textit{Value(e)} using Equation \ref{eq:score} based on the $\cB_j$ to which $n$ belongs. After having obtained the scores for all the training datapoints, we can take top $f$ elements and form the subset.
\end{enumerate}
The intuition behind using nearest neighbour technique is that if the point $e$ (whose score is unknown) is distant from the nearest neighbour $n$ (among the set of known scored points) by a factor $\epsilon$, the change in cumulative loss $I_t$ for including $e$ in place of $n$ will also be bounded. Hence, we can compute the score of the element $e$ by using the information acquired from selection of checkpoints. Theorem \ref{th:score} illustrates the same.

Following point 2 above, in order to incorporate diversity into the subset, we propose an Algorithm \ref{algo:simset}, \textit{SimSet} which computes the similarity values between a pair of instances based on their influences/contributions on the test set performance and retains the non-redundant and important training points. From Equation \ref{eq:finalapp2}, we can form the contribution score for each training datapoint $z_j^i$ as follows:
\begin{align}
    contrib(z_j^i) = \frac{1}{|\cB_j|} (\alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2])
\end{align}

\begin{align}
\label{eqn:optim}
    \min_{p_{ij}} & \sum_{i,j=1}^{|Z'|} p_{ij} \mathcal{D}_{ij} \\
    &s.t. \sum_{j=1}^{|Z'|} p_{i,j} = 1 , \nonumber \\
    &p_{i,j} \in [0,1] , \nonumber \\ 
    &\sum_{j=1}^{|Z'|}\| [p_{1,j} \dots p_{|Z'|,j} ] \|_2 \leq k
    \nonumber
\end{align}

\begin{algorithm}
 \caption{: SimSet}
 \label{algo:simset}
 \begin{algorithmic}
 \State \textbf{Input:}
 \State \hspace{2mm} Training dataset $\mathcal{Z}$ sorted based on obtained scores from Equation \ref{eq:score}, Subset size $k$
 \State \textbf{Output:}
 \State \hspace{2mm} Subset of training data $Z_S \subseteq \cZ$
 \State{\textbf{Algorithm:}}
 \hspace{2mm} $Z_S^0 =$ Initial set of top $k$ elements from $\mathcal{Z}$ based on scores.\\
 \hspace{2mm} Let $\mathcal{S} = $ cosine similarity of the pair $z_1,z_2\in \cZ$ as  $\cos(contrib(z_1), contrib(z_2)) $\\
 \hspace{2mm} Let $B_1,...,B_L$ be the top scoring elements of minibatches of $\cZ$ used for online subset selection. Compute similarities $\cS(Z_S^0,B_1),...,\cS(Z_S^0,B_L)$.
 \hspace{2mm}\For{each $B_l, l=1,...,L$ }\\
 \hspace{6mm}$Z' = Z_S^{l-1} \cup B_l$\\
 \hspace{6mm} Let $\mathcal{D}(z_1,z_2) = $ dissimilarity value for each pair $=1 - \cS(z_1,z_2)$ for every pair $(z_1, z_2) \in Z'$ ; $\mathcal{D} \in \mathcal{R}^{|Z'| \times |Z'|}$\\
 \hspace{6mm} $Z_S^l = $ Top $k$ representatives from $Z'$ using Equation \ref{eqn:optim}.
 \EndFor
 \end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{th:score}
Let $\cZ$ be the entire training set and $\cB$ be the minibatches associated with selected checkpoints $\in \mathcal{R}$. For each $e \in \cZ \setminus \cB$, if dist($e$,$n$) $\le \epsilon$, where $n$ is the nearest neighbour in terms of penultimate layer(PL) feature similarity ($PL_{\theta}(e)-PL_{\theta}(n) \le \epsilon$), the difference between cumulative change in loss on retaining $n (I_t)$ and substituting $e$ in place of $n (I_t')$ can be equated as 
\begin{equation}
    I_t' - I_t \le [f(e)_{g1}-f(n)_{g2}]
\end{equation}
where $f(n) = PL_{\theta}(n)^T FL_{\theta}$ with $FL_{\theta}$ being the final layer parameter, $f(e) = (PL_{\theta}(n)\pm \epsilon)^T FL_{\theta}$, and $g_1,g_2$ being the ground truth labels for $e$ and $n$ respectively.
\end{theorem}

% \subsection{Discussion}
% \textcolor{blue}{
% \begin{enumerate}
%     \item Both the phases of checkpoint selection and datapoint selection have to be in sync.
%     \item The score computation should match the approximation designed in the first phase.\\
%     Score ($z_j^i,z'$) = $\sum_{j\in \cS^t} \alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2] $
%     where $z_j^i \in z_j$ 
%     \item Extrapolation is required to compute the scores for the elements which do not belong to $z_j \forall j \in S$. Their representatives are found within $z_j$, and the corresponding scores are computed for those elements.
%     \item The Online OMP has to be designed such that two objectives are fulfilled: (a) Residual between $I_t$ and the selected checkpoints reduces. (b) The selected checkpoints should comprise of the datapoints/batches which form a good representative of the whole set.
% \end{enumerate}
% }


==> method1.tex <==

\newcommand{\tr}[1]{\textcolor{red}{#1}}

\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\RR}{\mathbb{R}}
\newtheorem{theorem}{Theorem}
% \title{Formulation Subset TracIn}
% \author{}
% \date{}
\section{Online Checkpoint Selection}
%Subset selection using data valuation is an efficient technique for filtering out the important training points necessary for explaining the predictions of a deep neural network model. 
In this section, we introduce the proposed data valuation method \textit{\ourmethod} -- a two-phase selection method using the training run of a gradient descent algorithm. The first phase selects informative checkpoints from the training algorithm, and  the second phase computes the value each datapoint. 
%Our novelty lies in the checkpoint selection obtaining which, we proceed to the next phase, datapoint selection, that is adapted from \cite{NEURIPS2020_e6385d39}.

\subsection{Data valuation using training trajectories}

We briefly review the TracIn \cite{NEURIPS2020_e6385d39} method.
Let $\mathcal{Z} = \{ z_i = (x_i , y_i)| i = 1,2,..,N\}$ be the training dataset for a supervised learning task with features $x_i \in \mathcal{X}$ and labels $y_i \in \mathcal{Y}$. Also, let $\mathcal{Z'} = \{ z'_j = (x'_j , y'_j)| j = 1,2,..,M\}$ be the valuation/test dataset which is used for assigning values/scores to a training datapoint $z\in \mathcal{Z}$. Additionally, let $\theta_1,...,\theta_T$ be a sequence of parameters generated by training with a given deep learning model on training dataset $\cZ$ using a mini-batch SGD-like algorithm.
TracIn \cite{NEURIPS2020_e6385d39} defines the scores for each training datapoint $z$, given a valuation datapoint $z'$ as the first order approximation for decrease in 
\begin{equation}
    l(\theta_{t+1},z') - l(\theta_t,z') =  \nabla l(\theta_t, z').(\theta_{t+1} - \theta_t)
\label{eqn:ap1}
\end{equation}
% $l(\theta_{t+1},z') - l(\theta_t,z') =  \nabla l(\theta_t, z').(\theta_{t+1} - \theta_t)$ 
where $l(\theta_t,z')$ is the loss(value function) on $z'$ using end-epoch model parameter $\theta_t$. The influence/score of any training point $z$ on the test set $\mathcal{Z'}$, being termed as \textit{TracIn}$(z,\mathcal{Z}')$ \cite{NEURIPS2020_e6385d39} uses parameters from uniformly selected end-epoch checkpoints $t = 1,2,..,T$ of a trained model and is defined as:
\begin{equation}
    TracIn(z,\mathcal{Z}') = \sum_{t=1}^T \nabla_{\theta_t} l (\theta_t, z).\nabla_{\theta_t} l (\theta_t, \mathcal{Z}')
\label{eq:tracin}
\end{equation}

We argue that the uniformly selected end-epoch checkpoints might not be a good measure for the above mentioned approximation since it does not consider the intermediate checkpoints while approximating $(\theta_{t+1} - \theta_t)$ (from first order) to $\nabla_{\theta_t} l (\theta_t, z)$, that shall be necessary in a mini-batch update setup. Hence, we propose a better approximation over the uniformly selected checkpoints.

\subsection{Proposed Approximation}
From first-order approximation of the value function (in this case test-set loss), we know
\begin{equation}
    l(\theta_{t+1},z') - l(\theta_t,z') =  \nabla l(\theta_t, z').(\theta_{t+1} - \theta_t)
\label{eqn:ap1}
\end{equation}

Assuming $\theta_{t}^0 = \theta_t$ and $\theta_{t}^O = \theta_{t+1}$ (total $O$ minibatches in epoch $t$), we can rewrite Equation \ref{eqn:ap1} as:

\begin{equation}
    \sum_{i=1}^O l(\theta_{t}^i,z') - l(\theta_{t}^{i-1},z') =  \sum_{i=1}^O (\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z')
\label{eqn:ap2}
\end{equation}

%where i denotes the batch number.

In this context, we adopt the 2nd order approximation where $(\nabla l(\theta_{t}^{i-1}, z'))^2$ is an approximate form of $\nabla^2 l(\theta_{t}^{i-1}, z')$. So we rewrite Equation \ref{eqn:ap2} as:

\begin{align}
    & \Vec{\triangle}_{t}(z') =
    \sum_{i=1}^O l(\theta_{t}^i,z') - l(\theta_{t}^{i-1},z') = \nonumber \\ & \sum_{i=1}^O (\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z') \nonumber \\ & + 0.5*((\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z'))^2
\label{eqn:ap2c}
\end{align}
where $\Vec{\triangle}_{t}(z')$ denotes change in test set loss over minibatches for epoch $t$.
% Let us call L.H.S of Eqn \ref{eqn:ap2c} as $\Vec{\triangle}_{t}(z')$ denoting change in test set loss over minibatches for epoch $t$:

% \begin{equation}
%     \Vec{\triangle}_{t} (z') = 
%     \sum_{i=1}^O l(\theta_{t}^i,z') - l(\theta_{t}^{i-1},z')
% \label{eqn:ap3}
% \end{equation}

%Let $\theta_{t}^{i}$ denote the SGD update.
Using the mini-batch weight update $\theta_{t}^{i} = \theta_{t}^{i-1} - \eta \nabla l(\theta_{t}^{i-1},z_i)$ , we can rewrite Equation \ref{eqn:ap2c} as: 

% \begin{equation}
%      \Vec{\triangle}_{t} (z') \approx \sum_{i=1}^O (\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z') + \nonumber \\ 0.5*((\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z'))^2
% \label{eqn:ap5}
% \end{equation}

% Using the update in Equation \ref{eqn:ap5}, we get:
\begin{align}
    \Vec{\triangle}_{t} (z') \approx -\eta \sum_{i=1}^O \nabla l(\theta_{t}^{i-1},z_i)^T \nabla l(\theta_{t}^{i-1}, z') \nonumber \\  + 0.5*(\nabla l(\theta_{t}^{i-1},z_i)^T \nabla l(\theta_{t}^{i-1}, z'))^2 \nonumber \\ \approx -\eta \sum_{i=1}^O \Vec{\mathcal{C}}_{i}^t(z_{i},z')
\label{eqn:ap6}
\end{align}

where $\Vec{\mathcal{C}}^{t}(z_{i},z')$ denotes the contribution of $z_{i}$ on $z'$ at epoch $t$ or similarity in gradients. $\Vec{\triangle}_{t} (z')$ is of the size $|$test set size$| \times$ 1 , while $\Vec{\mathcal{C}}^{t}(z,z')$ is of the size $|$test set size$| \times$ O

Mapping it to Orthogonal Matching Pursuit (OMP) problem where we want to form a set S containing $k$ out of $O$ checkpoints, the objective function comes to:

\begin{equation}
    \min ||\sum_{i \in S_{t}}({\alpha_i \Vec{\mathcal{C}}_{i}^t(z_i,z')}) - \Vec{\triangle}_{t}(z')||_2 \hspace{3mm} s.t. ||\alpha||_0 \leq k
\end{equation}

However, we propose to perform the selection in an online manner across epochs during the training. Hence, we propose an online version of OMP for selection of $k$ checkpoints.

\subsection{Phase 1: OMP based checkpoint selection}
\label{sec:oomp}

Consider the cumulative $\Delta_t$ vector that denotes the cumulative change in loss across epochs, 
$$I_t = \sum_{j=1}^t \Delta_j\ \ \forall t=1,...,T$$
% Also, let $C^t_i \in \RR^M \forall i\in \{1,...,O\}$, where $O$ is the number of number of batches in each epoch. 

In the online setting, at time $t$ we want to approximate:
$$ I_t \approx \sum_{j\in \cR^t} \alpha_j S^t_j $$ where, $\cS$ is the set having the gradient similarities of selected minibatches over time ad $\cR$ is the set of selected checkpoint/minibatch indices. So $\cS$ is of the size $|$test set size$| \times$ k. So, from Equation \ref{eqn:ap6}, we can rewrite the above approximation as:\\
\begin{align}
\label{eq:finalapp}
     I_t \approx \eta \sum_{j\in \cR^t} \alpha_j [\nabla l(\theta_{t}^{j-1},z_j)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j)^T \nabla l(\theta_{t}^{j-1}, z'))^2] 
\end{align\label{sec:method}}



The idea is to keep track of the selected checkpoints over time, and replace them with incoming checkpoints, based on their projections with the residual, which is the difference between the obtained estimate ($\xi = \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i$) and the ground truth ($I^t$ in this case). The detailed description is provided in Algorithm \ref{algo:onlineomp} and \ref{algo:replace}. 

% \textcolor{red}{Note for thought: Tweaking Online OMP algorithm to approximate the extrapolation during data valuation in Phase 2}
% Having obtained the set of checkpoints $S$, we compute the scores for each training point $z_i$ using the approximated estimate $\sum_{j\in \cS} \alpha_j S_j$.

 \begin{minipage}{0.46\textwidth}
 \begin{algorithm}[H]
 \caption{: OnlineCP}
 \label{algo:onlineomp}
 %\scriptsize
 %\label{algo:onlineomp}
 \begin{algorithmic}[1]
\State{\textbf{Input}:} $k$: Total number of checkpoints to be selected\\
$I$: Cumulative change in loss;
$C$: Gradient similarity

 \State \textbf{Initialize:}
 Set of selected components from C: $\cS$ = $\phi$\\
 Set of weights for the selected components: $\alpha = zero_{|S|}$ \\
 Estimate $\xi = \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i$, initially 0
%  Let the estimate $\xi = 0$ be the running estimate defined as $\sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i $ where $\alpha_i\in \alpha$ and $S_i\in \cS$
 
 \For{t = 1,...,T}
 \State \textbf{Input:} $I_t, C_i^t , \forall i\in\{1,...,O\} , ||C_i||_2 = 1 $
 \State{\textbf{Process}:}
 \State  Update $\alpha : argmin_\alpha \|\sum_{i \in |S|}(\alpha_i S_i) - I^t||_2$
 \State Update $\xi : \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i$
% \State $est = \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i $
% \State $res = I^t - est$
 \For{each batch $i \in O$:}
 \State ** Replacing selected checkpoints **
 \If{$|\cS| = k$}
 \State $\cS , \alpha, \xi$ = \textbf{Replace($I^t , \xi, \cS, \alpha , C_i^t$)}
 \Else
 \State ** Add the checkpoints sequentially **
 \State  $\cS \longleftarrow \cS \cup \{C_i^t\}$
 \State  Update $\alpha$ ; Update $\xi$
 \EndIf
 \EndFor
 \EndFor
 \State \textbf{Output}:Final set of selected checkpoints , $\cS$
 \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
 %\scriptsize
 \caption{: \textbf{Replace ($I^t , \xi, \cS, \alpha , C_i^t$)}}
 \label{algo:replace}
 \begin{algorithmic}[1]
\State  $\rho = I^t - \xi$ \*//Residual
 \State $maxproj = -\infty$ \*// best projection from existing set
 \State $ind = \phi$ \* /index of the best projection from existing set
 \For{each index $j$ in $\cS$:}
 %\State If{$|\cS| = k$}
 \State  $n\rho = \rho + \alpha_j*S_j$ \*// new residual on including $S_j$
 \State  $n\varrho = C_i^t . n\rho$  \*//projection of $C_i^t$ , incoming gradient
 \State  $\varrho = S_j . n\rho$  \*//projection of $S_j$, existing gradient
  \If{$n\varrho > \varrho$ and $n\varrho>maxproj$}
 \State maxproj $\longleftarrow$  $\varrho$
 \State $ind = j$
 \EndIf
 \EndFor
 \If{$ind \neq \phi$}
%  \State $S_{ind} \longleftarrow C_i^t$  \*//Replace $S_{ind}$ with $C_i^t$ which has higher projection than the best in set S: $S_{ind}$
 \State $S_{ind} \longleftarrow C_i^t$  \*//Replace the best existing projection in $S$ with the new projection
  \State Update $\alpha$ ; Update $\xi$
 \EndIf \\
 return $\cS, \alpha, \xi$
 \end{algorithmic}
\end{algorithm}
% \begin{algorithm}[H]
%  \scriptsize
%  \caption{: \textbf{Replace ($I^t , \xi, \cS, \alpha , C_i^t$)}}
%  \label{algo:replace}
%  \begin{algorithmic}[1]
% \State  $\rho = I^t - \xi$ \*//Residual
%  \State $maxproj = -\infty$ \*// best projection from existing set
%  \State $ind = \phi$ \* /index of the best projection from existing set
%  \For{each index $j$ in $\cS$:}
%  %\State If{$|\cS| = k$}
%  \State  $n\rho = \rho + \alpha_j*S_j$ \*// new residual on including $S_j$
%  \State  $n\varrho = C_i^t . n\rho$  \*//projection of $C_i^t$ , incoming gradient
%  \State  $\varrho = S_j . n\rho$  \*//projection of $S_j$, existing gradient
%   \If{$n\varrho > \varrho$ and $n\varrho>maxproj$}
%  \State maxproj $\longleftarrow$  $\varrho$
%  \State $ind = j$
%  \EndIf
%  \EndFor
%  \If{$ind \neq \phi$}
% %  \State $S_{ind} \longleftarrow C_i^t$  \*//Replace $S_{ind}$ with $C_i^t$ which has higher projection than the best in set S: $S_{ind}$
%  \State $S_{ind} \longleftarrow C_i^t$  \*//Replace the best existing projection in $S$ with the new projection
%   \State Update $\alpha$ ; Update $\xi$
%  \EndIf \\
%  return $\cS, \alpha, \xi$
%  \end{algorithmic}
% \end{algorithm}
\end{minipage}
\subsection{Phase 2: Data valuation using selected checkpoints}

The final approximation is demonstrated in Equation \ref{eq:finalapp} where $\cS$ contains the gradient similarity values w.r.t selected checkpoints. We can also rewrite Equation \ref{eq:finalapp} as:
\begin{align}
\label{eq:finalapp2}
     I_t \approx \eta \sum_{j\in \cR^t} \frac{1}{|\cB_j|} \sum_{i\in \cB_j} \alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2] 
\end{align}

where $\cB_j$ is the mini-batch associated with the selected checkpoint j $\in \cR$ and $z_j^i \in \cB_j$ is the i-th datapoint in $\cB_j$.
We associate the similarity in gradients (Equation \ref{eq:finalapp2}) to score/data value of the training points $\in \cB$ since that denotes the impact of the training point on the test set performance. We define the score in Equation \ref{eq:score}.

\begin{align}
\label{eq:score}
Value(z_j^i \in \cB_j) = \frac{1}{|\cB_j|} \sum_{z' \in \cZ'} (\alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2])
\end{align}

In order to select a subset of a given cardinality $f$, we can follow some techniques given below: 
\begin{enumerate}
    \item If $f < |\cB|$, where $|\cB|$ = $\sum_{j \in \cR} |\cB_j|$, we can take the top $f$ elements from $\cB$ in order of their scores obtained from Equation \ref{eq:score}.
    %\item Otherwise, we can take all the elements from $\cB$ and choose $f-|\cB|$ elements randomly from $\cZ \setminus \cB$.
    \item Otherwise, for $f > |B|$ we % form clusters with the selected elements $\in \cB$ (using feature values from trained model) and 
    find the nearest neighbouring point $n \in \cB$ (using some form of feature similarity) for each element $e$ in $\cZ \setminus \cB$. Following that, we can
    % either assign \textit{Value(e)} = \textit{Value(n)} , or 
    compute \textit{Value(e)} using Equation \ref{eq:score} based on the $\cB_j$ to which $n$ belongs. After having obtained the scores for all the training datapoints, we can take top $f$ elements and form the subset.
\end{enumerate}
The intuition behind using nearest neighbour technique is that if the point $e$ (whose score is unknown) is distant from the nearest neighbour $n$ (among the set of known scored points) by a factor $\epsilon$, the change in cumulative loss $I_t$ for including $e$ in place of $n$ will also be bounded. Hence, we can compute the score of the element $e$ by using the information acquired from selection of checkpoints. Theorem \ref{th:score} illustrates the same.

Following point 2 above, in order to incorporate diversity into the subset, we propose an Algorithm \ref{algo:simset}, \textit{SimSet} which computes the similarity values between a pair of instances based on their influences/contributions on the test set performance and retains the non-redundant and important training points. From Equation \ref{eq:finalapp2}, we can form the contribution score for each training datapoint $z_j^i$ as follows:
\begin{align}
    contrib(z_j^i) = \frac{1}{|\cB_j|} (\alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2])
\end{align}

\begin{align}
\label{eqn:optim}
    \min_{p_{ij}} & \sum_{i,j=1}^{|Z'|} p_{ij} \mathcal{D}_{ij} \\
    &s.t. \sum_{j=1}^{|Z'|} p_{i,j} = 1 , \nonumber \\
    &p_{i,j} \in [0,1] , \nonumber \\ 
    &\sum_{j=1}^{|Z'|}\| [p_{1,j} \dots p_{|Z'|,j} ] \|_2 \leq k
    \nonumber
\end{align}

\begin{algorithm}
 \caption{: SimSet}
 \label{algo:simset}
 \begin{algorithmic}
 \State \textbf{Input:}
 \State \hspace{2mm} Training dataset $\mathcal{Z}$ sorted based on obtained scores from Equation \ref{eq:score}, Subset size $k$
 \State \textbf{Output:}
 \State \hspace{2mm} Subset of training data $Z_S \subseteq \cZ$
 \State{\textbf{Algorithm:}}
 \hspace{2mm} $Z_S^0 =$ Initial set of top $k$ elements from $\mathcal{Z}$ based on scores.\\
 \hspace{2mm} Let $\mathcal{S} = $ cosine similarity of the pair $z_1,z_2\in \cZ$ as  $\cos(contrib(z_1), contrib(z_2)) $\\
 \hspace{2mm} Let $B_1,...,B_L$ be the top scoring elements of minibatches of $\cZ$ used for online subset selection. Compute similarities $\cS(Z_S^0,B_1),...,\cS(Z_S^0,B_L)$.
 \hspace{2mm}\For{each $B_l, l=1,...,L$ }\\
 \hspace{6mm}$Z' = Z_S^{l-1} \cup B_l$\\
 \hspace{6mm} Let $\mathcal{D}(z_1,z_2) = $ dissimilarity value for each pair $=1 - \cS(z_1,z_2)$ for every pair $(z_1, z_2) \in Z'$ ; $\mathcal{D} \in \mathcal{R}^{|Z'| \times |Z'|}$\\
 \hspace{6mm} $Z_S^l = $ Top $k$ representatives from $Z'$ using Equation \ref{eqn:optim}.
 \EndFor
 \end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{th:score}
Let $\cZ$ be the entire training set and $\cB$ be the minibatches associated with selected checkpoints $\in \mathcal{R}$. For each $e \in \cZ \setminus \cB$, if dist($e$,$n$) $\le \epsilon$, where $n$ is the nearest neighbour in terms of penultimate layer(PL) feature similarity ($PL_{\theta}(e)-PL_{\theta}(n) \le \epsilon$), the difference between cumulative change in loss on retaining $n (I_t)$ and substituting $e$ in place of $n (I_t')$ can be equated as 
\begin{equation}
    I_t' - I_t \le [f(e)_{g1}-f(n)_{g2}]
\end{equation}
where $f(n) = PL_{\theta}(n)^T FL_{\theta}$ with $FL_{\theta}$ being the final layer parameter, $f(e) = (PL_{\theta}(n)\pm \epsilon)^T FL_{\theta}$, and $g_1,g_2$ being the ground truth labels for $e$ and $n$ respectively.
\end{theorem}

% \subsection{Discussion}
% \textcolor{blue}{
% \begin{enumerate}
%     \item Both the phases of checkpoint selection and datapoint selection have to be in sync.
%     \item The score computation should match the approximation designed in the first phase.\\
%     Score ($z_j^i,z'$) = $\sum_{j\in \cS^t} \alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2] $
%     where $z_j^i \in z_j$ 
%     \item Extrapolation is required to compute the scores for the elements which do not belong to $z_j \forall j \in S$. Their representatives are found within $z_j$, and the corresponding scores are computed for those elements.
%     \item The Online OMP has to be designed such that two objectives are fulfilled: (a) Residual between $I_t$ and the selected checkpoints reduces. (b) The selected checkpoints should comprise of the datapoints/batches which form a good representative of the whole set.
% \end{enumerate}
% }


==> method2.tex <==

\newcommand{\tr}[1]{\textcolor{red}{#1}}

\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\RR}{\mathbb{R}}
\newtheorem{theorem}{Theorem}
% \title{Formulation Subset TracIn}
% \author{}
% \date{}
\section{Online Checkpoint Selection for Data Valuation}
\label{sec:method}
%Subset selection using data valuation is an efficient technique for filtering out the important training points necessary for explaining the predictions of a deep neural network model. 
In this section, we introduce the proposed data valuation method \textit{\ourmethod} -- a two-phase selection method using the training run of a gradient descent algorithm. The first phase selects informative checkpoints from the training algorithm, and  the second phase computes the value each datapoint. 
%Our novelty lies in the checkpoint selection obtaining which, we proceed to the next phase, datapoint selection, that is adapted from \cite{NEURIPS2020_e6385d39}.

\subsection{Data valuation using training trajectories}

We briefly review the TracIn \cite{NEURIPS2020_e6385d39} method.
Let $\mathcal{Z} = \{ z_i = (x_i , y_i)| i = 1,2,..,N\}$ be the training dataset for a supervised learning task with features $x_i \in \mathcal{X}$ and labels $y_i \in \mathcal{Y}$. Also, let $\mathcal{Z'} = \{ z'_j = (x'_j , y'_j)| j = 1,2,..,M\}$ be the valuation/test dataset which is used for assigning values/scores to a training datapoint $z\in \mathcal{Z}$. Additionally, let $\theta_1,...,\theta_T$ be a sequence of parameters generated by training with a given deep learning model on training dataset $\cZ$ using a mini-batch SGD-like algorithm.
TracIn \cite{NEURIPS2020_e6385d39} defines the scores for each training datapoint $z$, given a valuation datapoint $z'$ as the first order approximation for decrease in 
\begin{equation}
    l(\theta_{t+1},z') - l(\theta_t,z') =  \nabla l(\theta_t, z').(\theta_{t+1} - \theta_t)
\label{eqn:ap1}
\end{equation}
% $l(\theta_{t+1},z') - l(\theta_t,z') =  \nabla l(\theta_t, z').(\theta_{t+1} - \theta_t)$ 
where $l(\theta_t,z')$ is the loss(value function) on $z'$ using end-epoch model parameter $\theta_t$. The influence/score of any training point $z$ on the test set $\mathcal{Z'}$, being termed as \textit{TracIn}$(z,\mathcal{Z}')$ \cite{NEURIPS2020_e6385d39} uses parameters from uniformly selected end-epoch checkpoints $t = 1,2,..,T$ of a trained model and is defined as:
\begin{equation}
    TracIn(z,\mathcal{Z}') = \sum_{t=1}^T \nabla_{\theta_t} l (\theta_t, z).\nabla_{\theta_t} l (\theta_t, \mathcal{Z}')
\label{eq:tracin}
\end{equation}

We argue that the uniformly selected end-epoch checkpoints might not be a good measure for the above mentioned approximation since it does not consider the intermediate checkpoints while approximating $(\theta_{t+1} - \theta_t)$ (from first order) to $\nabla_{\theta_t} l (\theta_t, z)$, that shall be necessary in a mini-batch update setup. Hence, we propose a better approximation over the uniformly selected checkpoints.
\textcolor{red}{Why TracIn does not give good approximation? - First order, SGD}

\subsection{Proposed Approximation}
From first-order approximation of the value function (in this case test-set loss), we know
\begin{equation}
    l(\theta_{t+1},z') - l(\theta_t,z') =  \nabla l(\theta_t, z').(\theta_{t+1} - \theta_t)
\label{eqn:ap1}
\end{equation}

Assuming $\theta_{t}^0 = \theta_t$ and $\theta_{t}^O = \theta_{t+1}$ (total $O$ minibatches in epoch $t$), we can rewrite Equation \ref{eqn:ap1} as:

\begin{equation}
    \sum_{i=1}^O l(\theta_{t}^i,z') - l(\theta_{t}^{i-1},z') =  \sum_{i=1}^O (\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z')
\label{eqn:ap2}
\end{equation}

%where i denotes the batch number.

In this context, we adopt the 2nd order approximation where $(\nabla l(\theta_{t}^{i-1}, z'))^2$ is an approximate form of $\nabla^2 l(\theta_{t}^{i-1}, z')$. So we rewrite Equation \ref{eqn:ap2} as:

\begin{align}
    & \Vec{\triangle}_{t}(z') =
    \sum_{i=1}^O l(\theta_{t}^i,z') - l(\theta_{t}^{i-1},z') = \nonumber \\ & \sum_{i=1}^O (\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z') \nonumber \\ & + 0.5*((\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z'))^2
\label{eqn:ap2c}
\end{align}
where $\Vec{\triangle}_{t}(z')$ denotes change in test set loss over minibatches for epoch $t$.
% Let us call L.H.S of Eqn \ref{eqn:ap2c} as $\Vec{\triangle}_{t}(z')$ denoting change in test set loss over minibatches for epoch $t$:

% \begin{equation}
%     \Vec{\triangle}_{t} (z') = 
%     \sum_{i=1}^O l(\theta_{t}^i,z') - l(\theta_{t}^{i-1},z')
% \label{eqn:ap3}
% \end{equation}

%Let $\theta_{t}^{i}$ denote the SGD update.
Using the mini-batch weight update $\theta_{t}^{i} = \theta_{t}^{i-1} - \eta \nabla l(\theta_{t}^{i-1},z_i)$ , we can rewrite Equation \ref{eqn:ap2c} as: 

% \begin{equation}
%      \Vec{\triangle}_{t} (z') \approx \sum_{i=1}^O (\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z') + \nonumber \\ 0.5*((\theta_{t}^i - \theta_{t}^{i-1}) \nabla l(\theta_{t}^{i-1}, z'))^2
% \label{eqn:ap5}
% \end{equation}

% Using the update in Equation \ref{eqn:ap5}, we get:
\begin{align}
    \Vec{\triangle}_{t} (z') \approx -\eta \sum_{i=1}^O \nabla l(\theta_{t}^{i-1},z_i)^T \nabla l(\theta_{t}^{i-1}, z') \nonumber \\  + 0.5*(\nabla l(\theta_{t}^{i-1},z_i)^T \nabla l(\theta_{t}^{i-1}, z'))^2 \nonumber \\ \approx -\eta \sum_{i=1}^O \Vec{\mathcal{C}}_{i}^t(z_{i},z')
\label{eqn:ap6}
\end{align}

where $\Vec{\mathcal{C}}^{t}(z_{i},z')$ denotes the contribution of $z_{i}$ on $z'$ at epoch $t$ or similarity in gradients. $\Vec{\triangle}_{t} (z')$ is of the size $|$test set size$| \times$ 1 , while $\Vec{\mathcal{C}}^{t}(z,z')$ is of the size $|$test set size$| \times$ O

Mapping it to Orthogonal Matching Pursuit (OMP) problem where we want to form a set S containing $k$ out of $O$ checkpoints, the objective function comes to:

\begin{equation}
    \min ||\sum_{i \in S_{t}}({\alpha_i \Vec{\mathcal{C}}_{i}^t(z_i,z')}) - \Vec{\triangle}_{t}(z')||_2 \hspace{3mm} s.t. ||\alpha||_0 \leq k
\end{equation}

However, we propose to perform the selection in an online manner across epochs during the training. Hence, we propose an online version of OMP for selection of $k$ checkpoints.

\subsection{Phase 1: OMP based checkpoint selection}
\label{sec:oomp}
\textcolor{red}{Why online OMP?}

Consider the cumulative $\Delta_t$ vector that denotes the cumulative change in loss across epochs, 
$$I_t = \sum_{j=1}^t \Delta_j\ \ \forall t=1,...,T$$
% Also, let $C^t_i \in \RR^M \forall i\in \{1,...,O\}$, where $O$ is the number of number of batches in each epoch. 

In the online setting, at time $t$ we want to approximate:
$$ I_t \approx \sum_{j\in \cR^t} \alpha_j S^t_j $$ where, $\cS$ is the set having the gradient similarities of selected minibatches over time ad $\cR$ is the set of selected checkpoint/minibatch indices. So $\cS$ is of the size $|$test set size$| \times$ k. So, from Equation \ref{eqn:ap6}, we can rewrite the above approximation as:\\
\begin{align}
\label{eq:finalapp}
     I_t \approx \eta \sum_{j\in \cR^t} \alpha_j [\nabla l(\theta_{t}^{j-1},z_j)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j)^T \nabla l(\theta_{t}^{j-1}, z'))^2] 
\end{align}



The idea is to keep track of the selected checkpoints over time, and replace them with incoming checkpoints, based on their projections with the residual, which is the difference between the obtained estimate ($\xi = \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i$) and the ground truth ($I^t$ in this case). The detailed description is provided in Algorithm \ref{algo:onlineomp} and \ref{algo:replace}. 

% \textcolor{red}{Note for thought: Tweaking Online OMP algorithm to approximate the extrapolation during data valuation in Phase 2}
% Having obtained the set of checkpoints $S$, we compute the scores for each training point $z_i$ using the approximated estimate $\sum_{j\in \cS} \alpha_j S_j$.

 \begin{minipage}{0.46\textwidth}
 \begin{algorithm}[H]
 \caption{: \textbf{CheckSel}}
 \label{algo:onlineomp}
 %\scriptsize
 %\label{algo:onlineomp}
 \begin{algorithmic}[1]
\State{\textbf{Input}:} $k$: Total number of checkpoints to be selected\\
$I$: Cumulative change in loss;
$C$: Gradient similarity

 \State \textbf{Initialize:}
 Set of selected components from C: $\cS$ = $\phi$\\
 Set of weights for the selected components: $\alpha = zero_{|S|}$ \\
 Estimate $\xi = \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i$, initially 0
%  Let the estimate $\xi = 0$ be the running estimate defined as $\sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i $ where $\alpha_i\in \alpha$ and $S_i\in \cS$
 
 \For{t = 1,...,T}
 \State \textbf{Input:} $I_t, C_i^t , \forall i\in\{1,...,O\} , ||C_i||_2 = 1 $
 \State{\textbf{Process}:}
 \State  Update $\alpha : argmin_\alpha \|\sum_{i \in |S|}(\alpha_i S_i) - I^t||_2$
 \State Update $\xi : \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i$
% \State $est = \sum_{i\in \{1,...,|\cS|\}} \alpha_i S_i $
% \State $res = I^t - est$
 \For{each batch $i \in O$:}
 \State ** Replacing selected checkpoints **
 \If{$|\cS| = k$}
 \State $\cS , \alpha, \xi$ = \textbf{CheckReplace($I^t , \xi, \cS, \alpha , C_i^t$)}
 \Else
 \State ** Add the checkpoints sequentially **
 \State  $\cS \longleftarrow \cS \cup \{C_i^t\}$
 \State  Update $\alpha$ ; Update $\xi$
 \EndIf
 \EndFor
 \EndFor
 \State \textbf{Output}:Final set of selected checkpoints , $\cS$
 \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
 %\scriptsize
 \caption{: \textbf{CheckReplace ($I^t , \xi, \cS, \alpha , C_i^t$)}}
 \label{algo:replace}
 \begin{algorithmic}[1]
\State  $\rho = I^t - \xi$ \*//Residual
 \State $maxproj = -\infty$ \*// best projection from existing set
 \State $ind = \phi$ \* /index of the best projection from existing set
 \For{each index $j$ in $\cS$:}
 %\State If{$|\cS| = k$}
 \State  $n\rho = \rho + \alpha_j*S_j$ \*// new residual on including $S_j$
 \State  $n\varrho = C_i^t . n\rho$  \*//projection of $C_i^t$ , incoming gradient
 \State  $\varrho = S_j . n\rho$  \*//projection of $S_j$, existing gradient
  \If{$n\varrho > \varrho$ and $n\varrho>maxproj$}
 \State maxproj $\longleftarrow$  $\varrho$
 \State $ind = j$
 \EndIf
 \EndFor
 \If{$ind \neq \phi$}
%  \State $S_{ind} \longleftarrow C_i^t$  \*//Replace $S_{ind}$ with $C_i^t$ which has higher projection than the best in set S: $S_{ind}$
 \State $S_{ind} \longleftarrow C_i^t$  \*//Replace the best existing projection in $S$ with the new projection
  \State Update $\alpha$ ; Update $\xi$
 \EndIf \\
 return $\cS, \alpha, \xi$
 \end{algorithmic}
\end{algorithm}
% \begin{algorithm}[H]
%  \scriptsize
%  \caption{: \textbf{Replace ($I^t , \xi, \cS, \alpha , C_i^t$)}}
%  \label{algo:replace}
%  \begin{algorithmic}[1]
% \State  $\rho = I^t - \xi$ \*//Residual
%  \State $maxproj = -\infty$ \*// best projection from existing set
%  \State $ind = \phi$ \* /index of the best projection from existing set
%  \For{each index $j$ in $\cS$:}
%  %\State If{$|\cS| = k$}
%  \State  $n\rho = \rho + \alpha_j*S_j$ \*// new residual on including $S_j$
%  \State  $n\varrho = C_i^t . n\rho$  \*//projection of $C_i^t$ , incoming gradient
%  \State  $\varrho = S_j . n\rho$  \*//projection of $S_j$, existing gradient
%   \If{$n\varrho > \varrho$ and $n\varrho>maxproj$}
%  \State maxproj $\longleftarrow$  $\varrho$
%  \State $ind = j$
%  \EndIf
%  \EndFor
%  \If{$ind \neq \phi$}
% %  \State $S_{ind} \longleftarrow C_i^t$  \*//Replace $S_{ind}$ with $C_i^t$ which has higher projection than the best in set S: $S_{ind}$
%  \State $S_{ind} \longleftarrow C_i^t$  \*//Replace the best existing projection in $S$ with the new projection
%   \State Update $\alpha$ ; Update $\xi$
%  \EndIf \\
%  return $\cS, \alpha, \xi$
%  \end{algorithmic}
% \end{algorithm}
\end{minipage}
\subsection{Phase 2: Data valuation using selected checkpoints}

The final approximation is demonstrated in Equation \ref{eq:finalapp} where $\cS$ contains the gradient similarity values w.r.t selected checkpoints. We can also rewrite Equation \ref{eq:finalapp} as:
\begin{align}
\label{eq:finalapp2}
     I_t \approx \eta \sum_{j\in \cR^t} \frac{1}{|\cB_j|} \sum_{i\in \cB_j} \alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2] 
\end{align}

where $\cB_j$ is the mini-batch associated with the selected checkpoint j $\in \cR$ and $z_j^i \in \cB_j$ is the i-th datapoint in $\cB_j$.
We associate the similarity in gradients (Equation \ref{eq:finalapp2}) to score/data value of the training points $\in \cB$ since that denotes the impact of the training point on the test set performance. We define the score in Equation \ref{eq:score}.

\begin{align}
\label{eq:score}
Value(z_j^i \in \cB_j) = \frac{1}{|\cB_j|} \sum_{z' \in \cZ'} (\alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2])
\end{align}

In order to provide scores to all training data points, we find the nearest neighbouring point $n \in \cB$ (using some form of feature similarity) for each element $e$ in $\cZ \setminus \cB$. Following that, we can compute \textit{Value(e)} using Equation \ref{eq:score} based on the $\cB_j$ to which $n$ belongs.
% After having obtained the scores for all the training datapoints, we can take top $f$ elements and form the subset.
% In order to select a subset of a given cardinality $f$, we can follow some techniques given below: 
% \begin{enumerate}
%     \item If $f < |\cB|$, where $|\cB|$ = $\sum_{j \in \cR} |\cB_j|$, we can take the top $f$ elements from $\cB$ in order of their scores obtained from Equation \ref{eq:score}.
%     %\item Otherwise, we can take all the elements from $\cB$ and choose $f-|\cB|$ elements randomly from $\cZ \setminus \cB$.
%     \item Otherwise, for $f > |B|$ we % form clusters with the selected elements $\in \cB$ (using feature values from trained model) and 
%     find the nearest neighbouring point $n \in \cB$ (using some form of feature similarity) for each element $e$ in $\cZ \setminus \cB$. Following that, we can
%     % either assign \textit{Value(e)} = \textit{Value(n)} , or 
%     compute \textit{Value(e)} using Equation \ref{eq:score} based on the $\cB_j$ to which $n$ belongs. After having obtained the scores for all the training datapoints, we can take top $f$ elements and form the subset.
% \end{enumerate}
The intuition behind using nearest neighbour technique is that if the point $e$ (whose score is unknown) is distant from the nearest neighbour $n$ (among the set of known scored points) by a factor $\epsilon$, the change in cumulative loss $I_t$ for including $e$ in place of $n$ will also be bounded. Hence, we can compute the score of the element $e$ by using the information acquired from selection of checkpoints. Theorem \ref{th:score} illustrates the same.

In order to incorporate diversity into the subset, we define an objective function in Equation \ref{eqn:optim} that can be solved using Algorithm \ref{algo:simset}. It computes the similarity values between a pair of instances based on their influences/contributions (\textit{contrib)} and retains the non-redundant and important training points. From Equation \ref{eq:finalapp2}, we can form the contribution score for each training datapoint $z_j^i$ as follows:
\begin{align}
    contrib(z_j^i) = \frac{1}{|\cB_j|} (\alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') \nonumber \\ + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2])
\end{align}

\begin{align}
\label{eqn:optim}
    \min_{p_{ij}} & \sum_{i,j=1}^{|Z'|} p_{ij} \mathcal{D}_{ij} \\
    &s.t. \sum_{j=1}^{|Z'|} p_{i,j} = 1 , \nonumber \\
    &p_{i,j} \in [0,1] , \nonumber \\ 
    &\sum_{j=1}^{|Z'|}\| [p_{1,j} \dots p_{|Z'|,j} ] \|_2 \leq f
    \nonumber
\end{align}

\begin{algorithm}
 \caption{: Simsel}
 \label{algo:simset}
 \begin{algorithmic}
 \State \textbf{Input:}
 \State \hspace{2mm} Training dataset $\mathcal{Z}$ sorted based on obtained scores from Equation \ref{eq:score}, Subset size $f$
 \State \textbf{Output:}
 \State \hspace{2mm} Subset of training data $Z_S \subseteq \cZ$
 \State{\textbf{Algorithm:}}\\
 \hspace{2mm} $Z_S^0 =$ Top $f$ elements from $\mathcal{Z}$ based on scores.\\
 \hspace{2mm} $\mathcal{S} = $   $\cos(contrib(z_1), contrib(z_2)) $ where $z_1,z_2 \in \cZ$\\
 \hspace{2mm} Let $B_1,...,B_L$ be the minibatches of $\cZ$. 
%  Compute similarities $\cS(Z_S^0,B_1),...,\cS(Z_S^0,B_L)$.
 \hspace{2mm}\For{each $B_l, l=1,...,L$ }\\
 \hspace{6mm}$Z' = Z_S^{l-1} \cup B_l$\\
 \hspace{6mm} Let $\mathcal{D}(z_1,z_2) =1 - \cS(z_1,z_2)$ for every pair $(z_1, z_2) \in Z'$ ; $\mathcal{D} \in \mathcal{R}^{|Z'| \times |Z'|}$\\
 \hspace{6mm} $Z_S^l = $ Top $f$ representatives from $Z'$ (Equation \ref{eqn:optim}).
 \EndFor
 \end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{th:score}
Let $\cZ$ be the entire training set and $\cB$ be the minibatches associated with selected checkpoints $\in \mathcal{R}$. For each $e \in \cZ \setminus \cB$, if dist($e$,$n$) $\le \epsilon$, where $n$ is the nearest neighbour in terms of penultimate layer(PL) feature similarity ($PL_{\theta}(e)-PL_{\theta}(n) \le \epsilon$), the difference between cumulative change in loss on retaining $n (I_t)$ and substituting $e$ in place of $n (I_t')$ can be equated as 
\begin{equation}
    I_t' - I_t \le [f(e)_{g1}-f(n)_{g2}]
\end{equation}
where $f(n) = PL_{\theta}(n)^T FL_{\theta}$ with $FL_{\theta}$ being the final layer parameter, $f(e) = (PL_{\theta}(n)\pm \epsilon)^T FL_{\theta}$, and $g_1,g_2$ being the ground truth labels for $e$ and $n$ respectively.
\end{theorem}

% \subsection{Discussion}
% \textcolor{blue}{
% \begin{enumerate}
%     \item Both the phases of checkpoint selection and datapoint selection have to be in sync.
%     \item The score computation should match the approximation designed in the first phase.\\
%     Score ($z_j^i,z'$) = $\sum_{j\in \cS^t} \alpha_j [\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z') + 0.5*(\nabla l(\theta_{t}^{j-1},z_j^i)^T \nabla l(\theta_{t}^{j-1}, z'))^2] $
%     where $z_j^i \in z_j$ 
%     \item Extrapolation is required to compute the scores for the elements which do not belong to $z_j \forall j \in S$. Their representatives are found within $z_j$, and the corresponding scores are computed for those elements.
%     \item The Online OMP has to be designed such that two objectives are fulfilled: (a) Residual between $I_t$ and the selected checkpoints reduces. (b) The selected checkpoints should comprise of the datapoints/batches which form a good representative of the whole set.
% \end{enumerate}
% }


==> related_old.tex <==
\section{Related Work}
Finding influential training datapoints or data valuation has become a recent research challenge in the context of deep learning. It finds its application in subset selection, providing explanations to predictions, diagnosing mislabelled examples and so on. There have been several works in the literature of data valuation encompassing influence functions \cite{koh2017understanding}, shapley values \cite{ghorbani2019data}, reinforcement learning \cite{yoon2020data}, differentiable convex programming \cite{10.1007/978-3-030-86520-7_41}, tracking training trajectories \cite{NEURIPS2020_e6385d39} and more. However, apart from \cite{koh2017understanding} and \cite{NEURIPS2020_e6385d39}, all the other above-mentioned techniques are expensive to be scaled on large datasets and models since they merge the training and scoring datapoints in a combined framework.

Trained model information is used in \cite{koh2017understanding} and \cite{NEURIPS2020_e6385d39} to score datapoints. While \cite{koh2017understanding} estimates the change in parameter $\theta$ by upweighting the datapoint $x_i$ by a small $\epsilon$ to evaluate its influence, \cite{NEURIPS2020_e6385d39} on the other hand, tracks the training trajectory and estimates the influence of the datapoints. Our work is in close proximity to \cite{NEURIPS2020_e6385d39} with the difference being in the tracking of trajectories. While \cite{NEURIPS2020_e6385d39} uses uniformly selected checkpoints to evaluate scores, we develop an algorithm to select checkpoints during the training procedure aimed to optimise a value function.

Several works on selection of data that are designed to optimise objective functions range from using convex approach \cite{das2021tmcoss}, to submodular optimisation \cite{mirzasoleiman2020coresets}, to orthogonal matching pursuit (OMP) algorithms \cite{killamsetty2021grad}. We have developed an online orthogonal matching pursuit algorithm for the selection of checkpoints. There have been few works on online OMP algorithms \cite{saad2021online} \cite{6319766}, which mainly add instances independent of past queried instances, in an online streaming setting. Our proposed online OMP, however tracks the already selected checkpoints to make an informed decision on the incoming ones. To the best of our knowledge, this is one of the first works to develop an algorithm for selection of checkpoints while tracking the training procedure, and use them to evaluate training datapoints. Selecting subsets \cite{mirzasoleiman2020coresets}, \cite{killamsetty2021grad},\cite{coleman2019selection} of datapoints from vision datasets have been done that aim at developing efficient training strategy by selecting points at regular epochs. In these cases, the trained models are most likely to encounter the entire training dataset in subsets during the training. However, in our setting, a small fraction of the top scoring datapoints that we obtain after selection of checkpoints, are used only to train the models that have no prior information about the task under consideration, turning out to be efficient and scalable.
 


% \# Data Valuation\\
% 1. TracIn\\
% 2. Influence Function\\
% 3. DVRL\\
% 4. Data Shapley\\
% 5. Coresets
% 6. Grad match
% 7. HOST-CP

% \# OMP\\
% 5. Online Orthogonal Matching Pursuit (https://arxiv.org/abs/2011.11117)\\
% 6. ONLINE SEARCH ORTHOGONAL MATCHING PURSUIT (https://ieeexplore.ieee.org/document/6319766)\\

% \# Domain Adaptation\\
% 7. Larger Norm More Transferable: An Adaptive Feature Norm Approach for
% Unsupervised Domain Adaptation\\
% % (https://openaccess.thecvf.com/content\_ICCV\_2019/papers/Xu\_Larger\_Norm\_More\_Transferable\_An\_Adaptive\_Feature\_Norm\_Approach\_for\_ICCV\_2019\_paper.pdf)
% 8. Learning Causal Representation for Training Cross-Domain Pose Estimator via Generative Interventions\\
% % (https://openaccess.thecvf.com/content/ICCV2021/papers/Zhang\_Learning\_Causal\_Representation\_for\_Training\_Cross-Domain\_Pose\_Estimator\_via\_Generative\_ICCV\_2021\_paper.pdf)
% 9. Few-shot Domain Adaptation by Causal Mechanism Transfer\\
% % (https://icml.cc/Conferences/2020/ScheduleMultitrack?event=5935)
% 10. Domain Generalization using Causal Matching 
% % (https://icml.cc/Conferences/2021/ScheduleMultitrack?event=8586)




